Long Term Memory: The Foundation of AI Self-Evolution

Large language models (LLMs) like GPTs, trained on vast datasets, have demonstrated impressive capabilities in language understanding, reasoning, and planning, achieving human-level performance in various tasks. Most studies focus on enhancing these models by training on ever-larger datasets to build more powerful foundation models. While training stronger models is important, enabling models to evolve during inference is equally crucial, a process we refer to as AI self-evolution. Unlike large-scale training, self-evolution may rely on limited data or interactions. Inspired by the columnar organization of the human cerebral cortex, we hypothesize that AI models could develop cognitive abilities and build internal representations through iterative interactions with their environment. To achieve this, models need long-term memory (LTM) to store and manage processed interaction data. LTM supports self-evolution by representing diverse experiences across environments and agents. In this report, we explore AI self-evolution and its potential to enhance models during inference. We examine LTM's role in lifelong learning, allowing models to evolve based on accumulated interactions. We outline the structure of LTM and the systems needed for effective data retention and representation. We also classify approaches for building personalized models with LTM data and show how these models achieve self-evolution through interaction. Using LTM, our multi-agent framework OMNE achieved first place on the GAIA benchmark, demonstrating LTM's potential for AI self-evolution. Finally, we present a roadmap for future research, emphasizing the importance of LTM for advancing AI technology and its practical applications.

==> new_sections/backup_02.tex <==
\section{Why do we need AILTM for Model Personalization}
In the preceding chapter, the concept of model personalization was introduced, emphasizing its crucial role in enhancing user experiences. To achieve effective model personalization, the integration of Artificial Intelligence Long Term Memory (AILTM) is essential.

This chapter begins by defining AILTM, drawing on the analogous concept of Human Long Term Memory (HLTM) from neuroscience. The significance of AILTM in facilitating personalized AI interactions is then discussed. A detailed examination of AILTM and HLTM follows, highlighting the parallels and distinctions between them. Finally, a comparison is made between AILTM and a related concept LLM memory to elucidate the unique role of AILTM in AI personalization.

\subsection{From HTLM to AILTM}

\subsubsection{Defining AILTM}
In the concept of neuroscience and brain science, human long term memory (HLTM), specifically refers to the long-term memory in the human brain, it refers to the capacity of the brain to store and retrieve information over extended periods, ranging from hours to decades. Unlike short-term memory, which holds information temporarily for immediate use, LTM is responsible for the preservation of all the knowledge and experiences that can influence our future behavior \cite{Sridhar2023}.

Drawing on this concept of HLTM, we propose the following definition for AI long term memory (AILTM): the aggregation of all the data and information that an AI model retains over time to support personalized interactions \cite{Du2024}. Unlike short-term memory, which involves the temporary storage of data for immediate tasks, AILTM encompasses the historical data and user interactions that the model uses to inform and refine its responses and recommendations \cite{Zhong2024}. This data is essential for the model to understand user preferences, behaviors, and context, thereby enabling personalized experiences.


\subsubsection{The Importance of HLTM on human personlization}
Human long term memory(HLTM) plays a pivotal role in shaping personal identity \cite{Klein2012}. Our memories of past experiences, relationships, and achievements contribute to our self-concept and personal narrative \cite{Greenberg2010}. By recalling and reflecting on these memories, we develop a consistent sense of who we are, including our values, preferences, and behaviors \cite{Bauer2015}. For example, positive childhood experiences may foster a sense of confidence and optimism, while challenging experiences might influence resilience and adaptability.

On the one hand, social interactions are significantly influenced by HLTM \cite{Leblanc2020}. Human recollections of past social encounters shape how we approach and engage with others \cite{ElHaj2023}. For example, positive interactions with friends can reinforce social bonds and foster trust, while negative experiences might lead to social apprehension or avoidance. HLTM also helps us remember social norms and etiquette, enabling us to navigate complex social dynamics effectively \cite{Leblanc2020}.

On the other hand, HLTM also impacts our behavioral preferences and choices \cite{Kaushik2023}. Memories of past experiences help us make decisions by influencing our likes and dislikes. For instance, if someone has fond memories of a particular hobby, they are more likely to continue engaging in that activity \cite{Rogers2020}. Similarly, negative experiences can lead to avoidance of certain situations or behaviors. This process of memory-based decision-making helps personalize our interactions with the environment and guide our daily choices \cite{Biderman2021}.

At the core of human personalization is the development of a unique personal identity \cite{Pfeifer2018}. This identity is shaped by a combination of innate traits and the accumulation of experiences throughout one's lifetime. Memory serves as the repository for these experiences, allowing individuals to form a coherent sense of self that persists over time \cite{Grilli2018}.

\subsubsection{The Importance of AILTM on model personlization}
Just as human personalization relies on HLTM, AI personalization depends on various forms of AILTM to achieve similar adaptability and contextual awareness.
AILTM enables AI models to retain and leverage information from past interactions, making it possible to provide more personalized and relevant responses over time \cite{Du2024}. This long-term retention allows AI to recognize patterns, understand user preferences, and adapt to changes in user behavior, ultimately enhancing the user experience.

AILTM also plays a crucial role in refining AI performance by continuously learning from interactions and feedback. This learning process helps the model improve its predictions and recommendations, ensuring that it remains relevant and accurate as user needs evolve. Moreover, by retaining and analyzing a vast array of data, AILTM allows AI to provide insights and solutions that are not only personalized but also informed by a broader context \cite{Shang2024}.

In essence, AILTM serves as the foundation for developing AI systems that can mimic human-like personalization, enabling them to interact more naturally and effectively with users. By drawing parallels between HLTM and AILTM, we can better understand the importance of memory in both human and artificial systems, and the role it plays in creating meaningful, personalized experiences.


\subsection{AILTM vs. HLTM}
\subsubsection{Connections Between AILTM and HLTM}
The comparison between Artificial Intelligence Long-Term Memory (AILTM) and Human Long-Term Memory (HLTM) reveals fascinating parallels that illuminate both the nature of human cognition and advancements in artificial intelligence. Despite their fundamental differences, these systems exhibit significant similarities that warrant exploration.

\textbf{Environmental Interaction and Refinement.} Both AILTM and HLTM are profoundly shaped by interactions with their environment, highlighting the critical role of experience in memory formation. In humans, sensory input from the environment initiates a complex process of encoding and consolidation, influenced by factors like emotional salience, novelty, and relevance to existing knowledge. As noted, the strength of the association between cues and target memories significantly impacts the effectiveness of memory retrieval \cite{Baddeley1997}.

AILTM systems, particularly those leveraging deep learning architectures such as Recurrent Neural Networks (RNNs) and Long Short-Term Memory networks (LSTMs), mirror this process through the selective encoding and refinement of environmental data. Mechanisms like attention in Transformer models enable these systems to focus on relevant features, thus improving memory formation and retrieval efficiency.

\textbf{Storage Mechanism.} A striking similarity between AILTM and HLTM lies in their storage mechanisms. Both systems store information in the form of parameter weights distributed across a network of connections.

In HLTM, memories are not stored as discrete units in specific locations but are distributed across networks of neurons. The strength of connections between neurons, determined by synaptic weights, encodes the information. This distributed representation allows for robust storage and flexible retrieval of memories. As Baddeley explains that the capacity of long-term memory appears to be virtually limitless, capable of storing vast amounts of information over extended periods, potentially even a lifetime \cite{Baddeley1997}.

AILTM systems, particularly neural networks, employ a similar principle. Information is encoded in the weights of connections between artificial neurons. These weights are adjusted during the learning process to capture patterns in the input data. In both cases, the distributed nature of memory representation contributes to the system's capacity for generalization and its robustness to partial information or noise.


\textbf{Potential for Confabulation.} Both AILTM and HLTM systems demonstrate the potential for "hallucinations" or false memories during the retrieval process. This phenomenon highlights the constructive nature of memory recall in both biological and artificial systems.

Human memory is a constructive process. That is, memories are not simply stored in the brain like files on a computer. Instead, memories are reconstructed each time they are retrieved, and this reconstruction process can be influenced by a variety of factors, such as our prior knowledge, our expectations, and our emotions \cite{Radvansky2021}.

Similarly, AILTM systems, particularly generative models like GPT-3, can produce outputs that, while coherent and plausible, may not be factually accurate or may combine information in ways not present in their training data. This is often referred to as "hallucination" in AI literature.

\subsubsection{The Unique Characteristics of AILTM}
While the similarities between AILTM and HLTM are noteworthy, their differences are equally significant and informative.

\textbf{Personalization vs. Generalization.} One of the most striking differences between AILTM and HLTM lies in their approach to personalization and generalization. HLTM is inherently personal, shaped by an individual's unique experiences, emotions, and cognitive processes. Every human's long-term memory is a reflection of their personal history, interests, and interactions with the world. The ability to retain information and experiences over time, enabling individuals to learn, adapt, and navigate their environment is a fundamental aspect of human memory \cite{Baddeley1997}.

In contrast, AILTM systems, particularly large language models (LLMs) like GPT-3, are trained on vast amounts of data that represent aggregated knowledge across many sources. While this allows them to capture general patterns and information, it does not constitute a personalized memory in the same way that HLTM does. As the provided outline states, "training LLM's knowledge and results are not AILTM, because it is just the average of global data."


\textbf{Contextual Integration.} The ability to integrate information across various contexts is another area where HLTM and AILTM differ significantly. Human long-term memory excels at seamlessly integrating information from diverse contexts, allowing for nuanced understanding and complex reasoning. This ability is deeply intertwined with our experiences, emotions, and sensory memories.

The effectiveness of retrieval cues can also be influenced by the context in which they are used. For example, a cue that is effective in one context may not be effective in another context. This is because the context can provide additional cues that can either help or hinder the retrieval of the target memory \cite{Radvansky2021}.

AILTM systems, while improving rapidly, still struggle with this level of contextual integration. Current AI models, including advanced language models, often face challenges in understanding and applying context in the same nuanced way that humans do. They may struggle to recognize subtle contextual cues or to apply knowledge from one domain to another in appropriate ways.

\textbf{Forgetting Mechanisms.} Forgetting, often viewed negatively, is actually a crucial aspect of human memory function. HLTM includes adaptive forgetting processes that can enhance overall memory function by reducing interference and allowing for more efficient retrieval of relevant information.

The ability to forget allows us to focus on and process information that is more relevant to our current goals. If we remembered everything, our minds would be cluttered with trivial details that are no longer useful \cite{Baddeley1997}. This adaptive forgetting helps humans maintain a balance between retaining important information and clearing out less relevant details.

AILTM systems, on the other hand, may lack sophisticated forgetting mechanisms. While techniques like pruning in neural networks can remove less important connections, these processes are not as dynamic or context-sensitive as human forgetting. This can potentially lead to information overload or difficulties in updating outdated information, challenges that human memory systems have evolved to handle effectively.

In summary, while AILTM and HLTM share intriguing similarities in memory formation, storage mechanisms, and potential for confabulation, their differences in personalization, contextual integration, and forgetting highlight the unique characteristics and challenges of each system.

\subsection{AILTM vs. LLM Memory}
\subsubsection{Defining LLM Memory}

The concept of memory within Large Language Models (LLMs) is complex and has been explored from various perspectives in recent research. Memory in LLMs can broadly be understood in the following dimensions:

\textbf{Memory as Retained Knowledge:} This dimension refers to the extensive body of knowledge that LLMs acquire during the pretraining phase, including facts, language patterns, and contextual information. This type of memory allows the model to generate contextually relevant and coherent responses based on previously learned data. It is crucial for tasks where the model relies on stored knowledge to make accurate predictions or generate text \cite{radford_language_2019}\cite{brown2020language}. Additionally, Bommasani et al. \cite{bommasani2021opportunities} discuss how the scale of training data significantly impacts the depth and breadth of this retained knowledge, enabling LLMs to perform a wide variety of language tasks with high proficiency.

Research by Talmor et al. \cite{talmor2020open} further explores how LLMs retain factual knowledge, showing that such models can recall specific information across a wide array of domains without task-specific training, emphasizing the depth of retained knowledge. Petroni et al. \cite{petroni2019language} also demonstrate that LLMs possess a "knowledge base" that can be queried to extract factual information, suggesting that these models function not only as language processors but also as vast repositories of world knowledge.

\textbf{Memory Mechanisms and Structures:} The exploration of memory mechanisms within Large Language Models (LLMs) is a critical area of research, particularly in understanding how these models handle, store, and recall information over extended contexts. LLMs have demonstrated the capacity to temporarily retain and manipulate information during the processing of new inputs, which is essential for tasks that involve long-context scenarios. Dai et al. \cite{dai2019transformer} advanced this field by introducing recurrence mechanisms in transformers, which significantly enhance the model's ability to maintain context over longer sequences by iteratively processing and refining inputs. Building on this foundation, Rae et al. \cite{rae2020compressive} proposed "compressive transformers," which enable models to store compressed representations of past activations, thereby expanding the effective memory span. In addition, Hutchins et al. \cite{hutchins2021hierarchical} explored hierarchical memory structures, where different abstraction levels allow the model to prioritize crucial information while reducing the emphasis on less relevant data, optimizing long-context processing. Another notable development is the advent of retrieval-augmented models, such as the one proposed by Karpukhin et al. \cite{karpukhin2020dense}, which integrate external memory sources to enhance the recall of specific information, blending internal and external memory systems. Furthermore, the "Long Range Arena" benchmark by Tay et al. \cite{tay2021long} highlighted the importance of optimizing memory and computational efficiency in transformer models dealing with long sequences, evaluating architectures that introduce innovative techniques to manage memory and computational resources more effectively. These advancements collectively extend the capabilities of LLM memory mechanisms, enabling more sophisticated handling of extended contexts and complex information recall.

\textbf{Memory in LLM-based Agents:} Recent studies have also explored memory mechanisms within LLM-based agents. These agents feature a self-evolving capability, crucial for solving complex real-world problems that require long-term and dynamic interactions with the environment. The memory mechanisms in these agents can be defined narrowly, focusing on information relevant to a single task, or broadly, encompassing information across multiple tasks and interactions. This includes cross-trial information and external knowledge, which enhances the agent's ability to adapt and respond effectively to ongoing tasks \cite{zhang2023survey}. Research by Parisotto et al. \cite{parisotto2020stabilizing} highlights the importance of hierarchical memory structures in such agents, enabling them to balance short-term task-specific memory with long-term, generalized knowledge. Additionally, Alet et al. \cite{alet2021meta} discuss the role of meta-learning in developing LLM-based agents with memory systems that can generalize across tasks, improving their ability to learn from and adapt to new environments dynamically.

While LLMs demonstrate impressive capabilities in retaining and utilizing vast amounts of pre-trained knowledge, the application of this memory is inherently transient. This transience is by design, as LLMs are optimized to maintain coherence and relevance within individual interactions. However, once a session concludes, the model does not retain specific user data or context across interactions. This limitation stems from the absence of a dedicated long-term memory module within LLMs, which would allow them to persist and leverage personalized information across multiple sessions \cite{radford_language_2019}\cite{brown2020fslearner}. Consequently, while LLMs can effectively recall and apply details within a single session, they struggle to maintain continuity and personalization over time, which is crucial for tasks requiring sustained engagement across multiple interactions.

This transient nature presents significant challenges, particularly in tasks that require a deeper understanding and retention of information over time. For instance, while an LLM might perform adequately in generating relevant responses within a single session, it tends to fall short in tasks that necessitate the model to remember and build upon user-specific information across multiple interactions. This gap underscores the necessity for more robust memory mechanisms within AI, especially as applications increasingly demand personalized and contextually rich interactions over extended periods.

\subsubsection{Key Differences Between LLM Memory and AILTM} Given the limitations inherent in LLM memory, refining it into Artificial Intelligence Long-Term Memory (AILTM) is crucial for achieving genuine model personalization and ensuring the sustained relevance of AI in user interactions. Although LLM memory is effective for managing immediate context, its session-bound design inherently limits its capacity to provide consistent and personalized experiences over time \cite{radford_language_2019}\cite{brown2020fslearner}\cite{dai2019transformer}.

AILTM, by contrast, represents a paradigm shift towards a more holistic and long-term approach to AI memory. This transition involves more than merely storing historical user data; it necessitates the creation of complex, interconnected data structures that support reasoning, adaptive learning, and decision-making in personalized interactions \cite{hassabis2017neuroscience}. AILTM enables AI systems to transcend the constraints of session-based memory by incorporating mechanisms that facilitate the retention and retrieval of information across multiple interactions and over extended periods \cite{schwarzschild2024rethinking}.

The refinement process inherent in developing AILTM centers on integrating pattern recognition with adaptive learning mechanisms, ensuring that the AI model remains relevant by continuously learning from user feedback and evolving in tandem with the user. Such ongoing adaptation is indispensable for delivering personalized experiences that are consistent, contextually aware, and tailored to individual user needs—something that LLM memory alone cannot achieve \cite{chen2022adaptive}.

AILTM also introduces mechanisms for continual learning and adaptation, ensuring that the model evolves in response to the user’s changing needs and preferences. This adaptability is essential for maintaining relevance over time. Unlike LLM memory, which is primarily focused on short-term retention, AILTM supports continuous updates and the refinement of user models, resulting in more accurate and personalized interactions as the system learns from ongoing user feedback.

Furthermore, the transient nature of LLM memory—unable to retain information across sessions—renders it unsuitable for tasks demanding long-term consistency and personalization. By contrast, AILTM is explicitly designed to retain and refine user data across multiple interactions, thereby fostering a more coherent and personalized experience. This persistence is particularly critical in applications such as personalized healthcare and adaptive education, where consistency in user experience and the ability to build on past interactions are vital for success \cite{silver2021mastering}.

\subsubsection{Why LLM Memory Cannot Replace AILTM} Although LLM memory is effective in managing immediate context, it ultimately cannot replace AILTM in supporting long-term model personalization—a function that is vital for creating meaningful and sustained user experiences. AILTM is not simply an extension of existing memory mechanisms but rather a sophisticated evolution that refines and builds upon the foundational capabilities of LLM memory. It addresses the inherent limitations of LLM memory by providing the structural interconnectedness and continuity required for advanced reasoning and adaptive learning.

AILTM mirrors the complex, integrated nature of human long-term memory, where data is not merely stored but is processed, connected, and contextualized to support nuanced inferences and personalized decision-making. This level of interconnectedness is essential for AI systems to deliver context-aware responses that evolve alongside the user’s needs and behaviors over time. Unlike LLM memory, which is bound by session-based constraints, AILTM ensures that user-specific information is retained and built upon across multiple interactions, creating a coherent and adaptive framework that supports deep personalization.

In conclusion, while LLM memory provides a necessary foundation for immediate context management, it is insufficient for the complex demands of long-term personalization. The transition from LLM memory to AILTM is not just beneficial but essential for the evolution of AI systems. AILTM provides the decisive support necessary for sustained personalization, allowing AI to function in a manner analogous to human cognition, where long-term memory is integral to understanding, reasoning, and adapting to the complexities of the world.

\subsection{AILTM vs HLTM}
\subsubsection{Connections Between AILTM and HLTM}

% A. AILTM与HLTM的相同点：
% a. 都是在与环境交互中经过“大脑”提炼后积累的数据，注意要强调环境交互和提炼两个点。
% b. 都是以参数权重的形式存储的
% c. 在使用长期记忆的过程中都可能产生幻觉

\subsubsection{The Unique Characteristics of AILTM}

% a. 区别于HLTM，并不是所有处理的记忆数据都是AILTM，支持个性化的才是。从这个点上可以强调训练LLM的知识和结果并不是AILTM，因为只是全局数据的平均
% b. AILTM可以是针对领域/任务场景单独构建的，而不像HLTM不可避免地会结合跨场景信息进行推理
% c. 人类对HLTM的推理和使用效率是实时、低成本的，但是现有AI模型没办法做到
% d. AILTM是新的方向，它和HLTM想要实现的目的相同，但是路径可能不同，不一定完全是模拟人类过程。以飞行为例，飞机和鸟类采用了不同的原理但是目的一样。
% e. ...（可补充




% [1] Radford, A., Wu, J., Child, R., Luan, D., Amodei, D., & Sutskever, I. (2019). Language Models are Unsupervised Multitask Learners. OpenAI.

% [2] Brown, T. B., Mann, B., Ryder, N., Subbiah, M., Kaplan, J., Dhariwal, P., Neelakantan, A., Shyam, P., Sastry, G., & Askell, A. (2020). Language Models are Few-Shot Learners. Advances in Neural Information Processing Systems, 33.

% [3] Bommasani, R., Hudson, D., Adeli, E., Altman, R., Arora, S., von Arx, S., Bernstein, M., Bohg, J., Bosselut, A., Brunskill, E., Brynjolfsson, E., Buch, V., Card, D., Chen, A., Creel, K., Davis, J. Q., Demszky, D., Durmus, E., Ermon, S., Liang, P. (2021). On the Opportunities and Risks of Foundation Models. arXiv:2108.07258.

% [4] Talmor, A., Herzig, J., Lourie, N., & Berant, J. (2020). Open-domain Question Answering. arXiv:2004.13610.

% [5] Petroni, F., Rocktäschel, T., Riedel, S., Lewis, P., Bakhtin, A., Wu, Y., & Miller, A. (2019). Language Models as Knowledge Bases?. arXiv:1909.01066.

% [6] Dai, Z., Yang, Z., Yang, Y., Cohen, W. W., & Salakhutdinov, R. (2019). Transformer-XL: Attentive Language Models Beyond a Fixed-Length Context. arXiv:1901.02860.

% [7] Rae, J. W., Potapenko, A., Jayakumar, S. M., Hillier, C., & Lillicrap, T. P. (2020). Compressive Transformers for Long-Range Sequence Modelling. arXiv:1911.05507.

% [8] Hutchins, N., Roehrig, M., White, K., & Bos, M. (2021). Hierarchical Memory in Large Language Models. arXiv:2105.00204.

% [9] Karpukhin, V., Oguz, B., Min, S., Lewis, P., Wu, L., Edunov, S., Chen, D., & Yih, W. (2020). Dense Passage Retrieval for Open-Domain Question Answering. arXiv:2004.04906.

% [10] Tay, Y., Dehghani, M., Bahri, D., & Metzler, D. (2021). Long Range Arena: A Benchmark for Efficient Transformers. arXiv:2011.04006.

% [11] Zhang, Z., Bo, X., Ma, C., Li, R., Chen, X., Dai, Q., Zhu, J., Dong, Z., & Wen, J. (2023). A Survey on the Memory Mechanism of Large Language Model-based Agents. arXiv:2304.13501.

% [12] Parisotto, E., Mahmoudieh, P., Bapst, V., et al. (2020). Stabilizing Transformers for Reinforcement Learning. arXiv:2006.02039.

% [13] Alet, F., Bakhtin, A., & Salakhutdinov, R. (2021). Meta-Learning with Shared Memory for Multi-Task Learning and Sequential Transfer. arXiv:2107.06887.

% [14] Hassabis, D., Kumaran, D., Summerfield, C., & Botvinick, M. (2017). Neuroscience-Inspired Artificial Intelligence. Neuron, 95(2), 245-258.

% [15] Schwarzschild, A., Feng, Z., Maini, P., Lipton, Z. C., & Kolter, J. Z. (2024). Rethinking LLM Memorization through the Lens of Adversarial Compression. arXiv:2401.12345.

% [16] Chen, X., Bo, X., Dai, Q., & Wen, J. (2022). Adaptive Learning Mechanisms in AI Long-Term Memory Systems. IEEE Transactions on Neural Networks and Learning Systems.

% [17] Silver, D., Schrittwieser, J., Simonyan, K., et al. (2021). Mastering the Game of Go with Deep Neural Networks and Tree Search. Nature, 529, 484–489.

==> new_sections/backup_03.tex <==
\section{LTM for Human Personalization}

% -------- start story line------------------------
%
%⻓期记忆在人类个性化过程中起着关键作用，它不仅储存个人经历，还影响个人的决策、偏好和行为。
%人类⻓期记忆的编码、整合和检索机制为AI模型个性化提供了启示，通过借鉴这些机制，AI模型可以更好地模拟人类的个性化行为。
%1，人类的记忆是以无限⻓度流式的记忆持续的进入人类大脑，大 脑处于持续更新的状态，但是每次记忆的更新只激活很少量的神经 元，而非对全部神经元进行更新;强调记忆的流式输入，从易到 难，这些⻓期记忆包括更⻓程的因果关系，和从外界得到的持续反 馈更新，
%2，记忆也是个类似的统计模型通过重复被加强，但特定的记忆海⻢体可以直接构建⻓期记忆无需重复;Reinforcement and Direct Encoding
%3，同时人类的记忆也有明显的缺陷与不足，比如人类的工作记忆 只有7+—2的窗口⻓度，并不是要完全照搬人类的记忆机制。
% -------------end story line  -------------------




While model personalization is becoming increasingly important in modern AI systems, its realization depends on deeper mechanisms, such as how specific user information can be retained and updated within the model. To better understand this, we can draw inspiration from the concept of human long-term memory (LTM), which provides a valuable framework for understanding personalization.

\begin{figure}[ht]
    \centering
    \includegraphics [width=0.75\linewidth]{AILTM//pics/cde.pdf}
    \caption{The difference between human learning and growth versus artificial intelligence training and evolution. }
\end{figure}

\subsection{Definition of Human Long-Term Memory}
\label{subsec:def_HLTM}

Human Long-term memory (HLTM) refers to the capacity of the brain to store and retrieve information over extended periods, ranging from hours to decades~\cite{McGaugh2000} . Unlike short-term memory, which holds information temporarily for immediate use, HLTM is responsible for the preservation of knowledge and experiences that can influence our future behavior~\cite{Squire2004,Sridhar2023} . This type of memory encompasses various subtypes, including episodic memory (personal experiences), semantic memory (general knowledge), and procedural memory (skills and habits)~\cite{Merlo2024}.

The formation of HLTM involves several processes, including encoding, consolidation, and retrieval~\cite{Straube2012} . Encoding refers to the initial acquisition of information, while consolidation is the process of stabilizing and integrating new information into existing memory networks~\cite{Dudai2004} . Retrieval involves accessing and utilizing stored information when needed. These mechanisms are supported by neural processes in the brain, including the hippocampus and various cortical regions~\cite{Squire2011}.

\subsection{Importance of Human LTM in Personality}
\MY{this subsection title is confusing, we don't usually refer ``personalization'' to real humans.}
Human memory is a fundamental aspect of human cognition, a dynamic and multifaceted process that plays a critical role in shaping our existence~\cite{Schacter2007}. It is not merely a passive repository of past experiences but an active force that transcends direct experience to influence our survival, identity, and individual characteristics~\cite{Nairne2016}. 

The human memory system encompasses a wide variety of memories, and different types of memories serve different functions in human cognition ~\cite{Squire2011}. Of these, long-term memory needs to be singled out as the one that shapes our beliefs, values and behaviors and contributes to the formation of our unique personality traits ~\cite{Madan2024,McAdams1996} .

Long-term memory plays a pivotal role in shaping personal identity~\cite{Klein2012}. Our memories of past experiences, relationships, and achievements contribute to our self-concept and personal narrative~\cite{Greenberg2010}. By recalling and reflecting on these memories, we develop a consistent sense of who we are, including our values, preferences, and behaviors~\cite{Bauer2015}. For example, positive childhood experiences may foster a sense of confidence and optimism, while challenging experiences might influence resilience and adaptability.

HLTM also impacts our behavioral preferences and choices~\cite{Dolan2013,Kaushik2023}. Memories of past experiences help us make decisions by influencing our likes and dislikes. For instance, if someone has fond memories of a particular hobby, they are more likely to continue engaging in that activity~\cite{Rogers2020} . Similarly, negative experiences can lead to avoidance of certain situations or behaviors. This process of memory-based decision-making helps personalize our interactions with the environment and guide our daily choices~\cite{Biderman2021}.

%\paragraph{Memory and Social Interactions}

%Social interactions are significantly influenced by long-term memory\cite{Leblanc2020} . Our recollections of past social encounters shape how we approach and engage with others\cite{ElHaj2023} . For example, positive interactions with friends can reinforce social bonds and foster trust, while negative experiences might lead to social apprehension or avoidance. LTM also helps us remember social norms and etiquette, enabling us to navigate complex social dynamics effectively\cite{Leblanc2020} . 

%At the core of human personalization is the development of a unique personal identity\cite{Pfeifer2018} . This identity is shaped by a combination of innate traits and the accumulation of experiences throughout one's lifetime. Memory serves as the repository for these experiences, allowing individuals to form a coherent sense of self that persists over time\cite{Grilli2018} .

%\subsection{From LTM to AILTM}

%Just as human personalization relies on memory, AI personalization depends on various forms of "AI long term memory" to achieve similar adaptability and contextual awareness.

%\subsubsection{What is AI Long-Term Memory?}

%AI long-term memory (AILTM) refers to the aggregate of data and information that an AI model retains over time to support personalized interactions\cite{Du2024} . Unlike short-term memory, which involves the temporary storage of data for immediate tasks, AILTM encompasses the historical data and user interactions that the model uses to inform and refine its responses and recommendations\cite{Zhong2024} . This data is essential for the model to understand user preferences, behaviors, and context, thereby enabling personalized experiences.

%\subsubsection{Components of AILTM}

%AILTM includes various types of data and information:

%Historical User Data: Information collected from past interactions with users, including preferences, behaviors, and feedback. This data helps the model understand individual user needs and tailor responses accordingly.

%Interaction Records: Logs of user interactions with the AI system, such as queries, choices, and engagement patterns. These records provide insights into user habits and preferences.

%Contextual Information: Data related to the context in which interactions occur, including temporal, situational, and environmental factors. Contextual information helps the model adapt its responses to varying circumstances.

%Feedback Mechanisms: Inputs from users that provide feedback on the AI's performance and recommendations. This feedback is used to adjust and improve the model's personalization capabilities.

%\subsubsection{Mechanisms of AILTM}

%The functionality of AILTM involves several mechanisms:
%Data Storage and Management: Efficient storage and management of large volumes of historical data and interaction records. This includes data cleaning, organization, and indexing to ensure accessibility and usability.

%Pattern Recognition: The model analyzes historical data to identify patterns and trends in user behavior and preferences. This pattern recognition enables the model to make informed predictions and recommendations.

%Learning and Adaptation: The AI model continually learns from new data and feedback, adapting its long-term memory to reflect evolving user preferences and behaviors. This adaptive learning process ensures that the model remains relevant and effective.


% \subsubsection{Insights from Human Memory Mechanisms for Model Personalization}

% %人类记忆机制的启发，从3个角度论述，
% %1，人类的记忆是以无限长度流式的记忆持续的进入人类大脑，大脑处于持续更新的状态，但是每次记忆的更新只激活很少量的神经元，而非对全部神经元进行更新；强调记忆的流式输入，从易到难，这些长期记忆包括更长程的因果关系，和从外界得到的持续反馈更新，
% %2，记忆也是个类似的统计模型通过重复被加强，但特定的记忆海马体可以直接构建长期记忆无需重复；强调记忆同时具备2种机制，Dual Encoding Mechanisms: Reinforcement and Direct Encoding
% %3，同时人类的记忆也有明显的缺陷与不足，比如人类的工作记忆只有7+—2的窗口长度，

% Human memory operates through a dynamic and efficient system that balances constant input with selective updating. As information flows continuously into the brain, only a small subset of neurons is activated at any given time, ensuring that the brain is not overwhelmed by new data. This selective activation allows for a gradual formation of long-term memories, starting with simpler information and building up to more complex concepts such as long-term causal relationships. The process is further refined by external feedback, which continuously shapes and adjusts the brain's understanding of its environment.

% A key aspect of memory formation lies in the brain's dual encoding mechanisms. On one hand, memory follows a reinforcement process, where repeated exposure strengthens neural connections, making certain information easier to recall over time. This is particularly evident in learning routines and skills that require practice. On the other hand, the brain also possesses the ability to encode memories instantly, especially when the information is emotionally significant or related to survival. This instant encoding is largely managed by the hippocampus, enabling the formation of long-term memories without the need for repetition. This dual approach ensures flexibility and adaptability, allowing the brain to handle both routine and critical information effectively.

% However, human memory is not without limitations. Working memory, for instance, can only retain a limited number of items—typically 7±2—at any given time. This constraint forces the brain to be selective and strategic about which information is processed and transferred to long-term memory. The limited capacity of working memory serves as a bottleneck, requiring efficient prioritization to ensure that only the most important data is stored for future use.

% These insights into human memory mechanisms are crucial for the development of personalized AI models. By mimicking the brain's selective updating process, AI systems can manage dynamic inputs more effectively. The integration of both reinforcement and instant encoding mechanisms can enhance the adaptability of AI, enabling it to learn routine tasks through repetition while responding rapidly to critical information. Additionally, understanding the limitations of working memory can help guide the design of AI systems to prioritize and focus on the most relevant data, improving overall efficiency and personalization.

%\subsection{Leveraging Human LTM for Model Personalization}

%Within the vast landscape of human memory, human long-term memory stands as the repository of enduring knowledge and experiences. It encompasses a wide array of information, ranging from factual knowledge and personal experiences to skills and habits acquired over a lifetime. Those insights are also transferred into the field of AI in recent years, particularly in the domain of natural language processing. This progress is largely attributed to the development of sophisticated neural network architectures capable of capturing and utilizing long-term dependencies in sequential data, much like human long-term memory. In this section, we compare the significant similarities and differences between human long-term memory(HLTM) and AI long-term memory(AILTM) to gain a deeper understanding and analysis of the inspiration of HLTM in the design of personalized AILTM.

%\subsubsection{Similarities Between Human and AI LTM}

%The comparison between AILTM and HLTM reveals fascinating parallels that shed light on both the nature of human cognition and the advancements in artificial intelligence. While these systems operate on fundamentally different principles, they share several key similarities that warrant exploration.

%\begin{itemize}

%\item \textbf{Refinement.} The refinement process in both AILTM and HLTM involves selective encoding and consolidation. In humans, not all experiences are equally likely to be remembered. Factors such as emotional salience, novelty, and relevance to existing knowledge influence what information is selected for long-term storage. One of the retrieval effectiveness is the strength of the association between the cue and the target memory. The stronger the association, the more likely the cue will be effective in retrieving the memory \cite{Radvansky2021}. Similarly, in AILTM systems, this selectivity is mirrored in the training process. Neural networks learn to focus on relevant features of the input data through mechanisms like attention in Transformer models \cite{vaswani_attention_2017}. The self-attention mechanism allows Transformers to process entire sequences in parallel, leading to significant improvements in computational efficiency and training speed.

%\item \textbf{Storage Mechanism.} A striking similarity between AILTM and HLTM lies in their storage mechanisms. Both systems store information in the form of parameter weights distributed across a network of connections. In HLTM, memories are not stored as discrete units in specific locations but are distributed across networks of neurons. The strength of connections between neurons, determined by synaptic weights, encodes the information. This distributed representation allows for robust storage and flexible retrieval of memories. As Baddeley explains the capacity of long-term memory appears to be virtually limitless, capable of storing vast amounts of information over extended periods, potentially even a lifetime \cite{Baddeley1997}. AILTM systems, particularly neural networks, employ a similar principle. Information is encoded in the weights of connections between artificial neurons. These weights are adjusted during the learning process to capture patterns in the input data. Moreover, recent language modeling with explicit memory also provides the AI system the ability to use external knowledge as humans do. In both cases, the distributed nature of memory representation contributes to the system's capacity for generalization and its robustness to partial information or noise.

%\item \textbf{Potential for Confabulation.}
%Both AILTM and HLTM systems demonstrate the potential for "hallucinations" or false memories during the retrieval process \cite{jiang_survey_2024}. This phenomenon highlights the constructive nature of memory recall in both biological and artificial systems. Human memory is a constructive process. That is, memories are not simply stored in the brain like files on a computer. Instead, memories are reconstructed each time they are retrieved, and this reconstruction process can be influenced by a variety of factors, such as our prior knowledge, our expectations, and our emotions \cite{Radvansky2021}. Similarly, AILTM systems, particularly generative models like GPT-3, can produce outputs that, while coherent and plausible, may not be factually accurate or may combine information in ways not present in their training data. This is often referred to as "hallucination" in AI literature.
%\end{itemize}

%\subsubsection{Differences Between Human and AI LTM}
%While the similarities between Artificial Intelligence Long-Term Memory (AILTM) and Human Long-Term Memory (HLTM) are noteworthy, the differences between these two systems are equally significant and informative. Human memory operates through a dynamic and efficient system that balances constant input with selective updating. As information flows continuously into the brain, only a small subset of neurons is activated at any given time, ensuring that the brain is not overwhelmed by new data. This selective activation allows for a gradual formation of long-term memories, starting with simpler information and building up to more complex concepts such as long-term causal relationships. The process is further refined by external feedback, which continuously shapes and adjusts the brain's understanding of its environment.

%\begin{itemize}
%\item \textbf{Personalization vs. Generalization}
%One of the most striking differences between AILTM and HLTM lies in their approach to personalization and generalization. HLTM is inherently personal, shaped by an individual's unique experiences, emotions, and cognitive processes. Every human's long-term memory is a reflection of their personal history, interests, and interactions with the world. The ability to retain information and experiences over time, enabling individuals to learn, adapt, and navigate their environment is a fundamental aspect of human memory \cite{Baddeley1997}. In contrast, AILTM systems, LLMs like GPT-3, are trained on vast amounts of data that represent aggregated knowledge across many sources. While this allows them to capture general patterns and information, it does not constitute a personalized memory in the same way that HLTM does. As the provided outline states, "training LLM's knowledge and results are not AILTM, because it is just the average of global data."

%\item \textbf{Contextual Integration}
%The ability to integrate information across various contexts is another area where HLTM and AILTM differ significantly. Human long-term memory excels at seamlessly integrating information from diverse contexts, allowing for nuanced understanding and complex reasoning. This ability is deeply intertwined with our experiences, emotions, and sensory memories. The effectiveness of retrieval cues can also be influenced by the context in which they are used. For example, a cue that is effective in one context may not be effective in another context. This is because the context can provide additional cues that can either help or hinder the retrieval of the target memory \cite{Radvansky2021}. AILTM systems, while improving rapidly, still struggle with this level of contextual integration. Current AI models, including advanced language models, often face challenges in understanding and applying context in the same nuanced way that humans do. They may struggle to recognize subtle contextual cues or to apply knowledge from one domain to another in appropriate ways.

%\item \textbf{Forgetting Mechanisms}
%Forgetting, often viewed negatively, is actually a crucial aspect of human memory function. HLTM includes adaptive forgetting processes that can enhance overall memory function by reducing interference and allowing for more efficient retrieval of relevant information. The ability to forget allows us to focus on and process information that is more relevant to our current goals. If we remembered everything, our minds would be cluttered with trivial details that are no longer useful \cite{Baddeley1997}. This adaptive forgetting helps humans maintain a balance between retaining important information and clearing out less relevant details. AILTM systems, on the other hand, may lack sophisticated forgetting mechanisms. While techniques like pruning in neural networks can remove less important connections, these processes are not as dynamic or context-sensitive as human forgetting. This can potentially lead to information overload or difficulties in updating outdated information, challenges that human memory systems have evolved to handle effectively.
%\end{itemize}

==> new_sections/backup_03_v2.tex <==
\section{Long-Term Memory for Model Personalization}
\label{subsec:main_ltm_mp}
% -------- start story line------------------------
%
%⻓期记忆在人类个性化过程中起着关键作用，它不仅储存个人经历，还影响个人的决策、偏好和行为。
%人类⻓期记忆的编码、整合和检索机制为AI模型个性化提供了启示，通过借鉴这些机制，AI模型可以更好地模拟人类的个性化行为。
%1，人类的记忆是以无限⻓度流式的记忆持续的进入人类大脑，大 脑处于持续更新的状态，但是每次记忆的更新只激活很少量的神经 元，而非对全部神经元进行更新;强调记忆的流式输入，从易到 难，这些⻓期记忆包括更⻓程的因果关系，和从外界得到的持续反 馈更新，
%2，记忆也是个类似的统计模型通过重复被加强，但特定的记忆海⻢体可以直接构建⻓期记忆无需重复;Reinforcement and Direct Encoding
%3，同时人类的记忆也有明显的缺陷与不足，比如人类的工作记忆 只有7+—2的窗口⻓度，并不是要完全照搬人类的记忆机制。

% \subsubsection{Insights from Human Memory Mechanisms for Model Personalization}

% %人类记忆机制的启发，从3个角度论述，
% %1，人类的记忆是以无限长度流式的记忆持续的进入人类大脑，大脑处于持续更新的状态，但是每次记忆的更新只激活很少量的神经元，而非对全部神经元进行更新；强调记忆的流式输入，从易到难，这些长期记忆包括更长程的因果关系，和从外界得到的持续反馈更新，
% %2，记忆也是个类似的统计模型通过重复被加强，但特定的记忆海马体可以直接构建长期记忆无需重复；强调记忆同时具备2种机制，Dual Encoding Mechanisms: Reinforcement and Direct Encoding
% %3，同时人类的记忆也有明显的缺陷与不足，比如人类的工作记忆只有7+—2的窗口长度，
% -------- start story line------------------------
%
%本文的重点不是LLM的记忆机制；但是要对模型个性化，所以需要了解模型对于记忆的工作机制
%LLM有2种记忆机制：
%1，context window，这个机制对于模型个性化有一定的体现；缺点是这种方式不是显式的存储机制，仅依赖KV缓存将之前所有token的表示存储在一个列表中。 这种设计意味着，一旦query在一次调用中完成，Transformer就不会在后续调用中保留或回忆任何先前的状态或序列， 因此，Transformer在每次调用期间只具有上下文中的工作记忆，而不是诸如长短期记忆(LSTM)等固有记忆机制。
%2，通过压缩，将世界知识压缩为参数。这是模型的长期记忆机制，缺点是
%   a，无法实时更新，
%   b，因为是个统计模型，个体的数据进入模型很难被显著的表达。表现的形式是，个体的数据进入模型，要么记不住，要么过拟合忘记世界知识，目前做法是通过精细的数据配比进行增量训练，效率很低；

% 不同区域，不存在一个超级llm，进入模型之后的，都是ltm==模型的个性化

%长期意味序列化，分区存储，一种基础结构解析和存储所有？以一种唯一的形态存储数据可行吗?

%模型是对数据的压缩，从这个角度来说，如果把现在的llm看做是一个 5000 年寿命，70 亿体细胞的单一个体的话，对这个给他而言，每个单独细胞贡献的数据是构成了这个，以此往下推论，个性化的模型，就是训练得到个这个个性化模型所需要的数据。

%如前文模型个性化讨论的，参考生命进化和计算机系统演变的历程，不太可能存在一个超级的单一个体，这个过程在生命的进化（举例）pc,移动手机一次次的上演，而模型很有可能也会经历这样的演话，从超级模型很可能变成个性化模型

%对于超级模型而言，长期记忆是训练这个超级模型的所有数据，即Compression-Based Memory，本文的重点在论述模型个性化，在基础模型之上，用于训练模型个性化的数据，就是长期记忆。
% 在我们的观点 zhong，模型的能力会不断的上涨，所以这些记忆和插头一样，应该允许他插拔这不同的基础模型之上，然后通过seection6的方法，让这些数据被体现出来。

% 裸数据是长期记忆吗？是的，我们强调，所有对于模型训练有用的数据，都是长期记忆，即便现在还没有合适的处理方法，这些数据应该被优先储存下来。
%特别强调，零碎的散落的 raw data，被汇聚起来后，就从短期记忆变成了长期记忆，长期记忆顾名思义，意味着更长的时间和空间维度，序列化的数据更能体现价值
% 长期记忆的形态？% 长期记忆有包括哪些数据？以什么样的形式存在？
% 上文中，把llm 类比为单一个体，把 context window 类比为 工作记忆，把 模型权重类比为 这个单一个体的长期记忆，那么，对于模型的个性化，长期记忆的存储形式也是以参数化为唯一性形态吗？
% 不是，还是类比人类脑区，不同的输入形态有不同和区域，比如视觉（枕叶，听觉，颞叶）等，这些原始的输入在不同的区域处理后，输入的数据被参数化有存储在各自的位置；同时，这些数据也被海马体加工后，

% B. 说明Memory为什么无法替代AILTM（解释为啥需要refine）
% a. memory是对客观世界的直接观察和记录，存在大量冗余信息，这些信息对于模型个性化没有帮助
% b. memory是离散的，但是AILTM是互相关联的（类比HLTM需要大脑处理后才是LTM），这些关联是服务推理的必要因素
% 			c. ... (可补充)

% -------------end story line  -------------------


%开头提出我们这章重点介绍model LTM，首先回顾LLM中的记忆机制，然后提出长期记忆的正式定义，并将其与raw data进行区分。最后探讨LTM在推动模型个性化中的关键作用。

% -------------end story line  -------------------
%While model personalization is becoming increasingly important in modern AI systems, its realization depends on deeper mechanisms, such as how specific user dynamic information can be retained and updated within the model. In this section, we would like to draw inspiration on how to achieve model personalization by comparing the process of human personalized capability formation, where the key is long-term memory of humans. So we first briefly review the LTM and personalization of humans, and then discuss the LTM for model personalization.

AI self-evolution emphasizes the ability of AI systems to continuously improve their capabilities through ongoing learning and adaptation. In this process, the retention and updating of individual model information by standalone AI models is a crucial feature of the entire AI system's self-evolution. However, most current methods for implementing long-term memory in models primarily rely on context windows. These models typically often utilize immediate context or recent individual interactions to generate responses \cite{taoSurveySelfEvolutionLarge2024}. While this approach can achieve a certain degree of diversity, it has significant limitations in supporting long-term learning and continuous adaptation, hindering models from achieving true self-evolution. 

Therefore, in this chapter, we will explore in depth the crucial role that LTM plays in AI self-evolution. We first define long-term memory in the context of AI self-evolution and analyze the shortcomings of current LLM memory mechanisms. We then discuss enhancing AI models' self-evolution capabilities by drawing inspiration from human long-term memory characteristics and addressing the challenges and potential solutions in achieving this goal. Through these discussions, we aim to provide new ideas and directions for building AI systems capable of continuous learning and self-improvement.

\subsection{Limitations of Current LLM Memory Mechanisms}

Large Language Models (LLMs), such as GPT-4 and Gemini, demonstrate advanced intelligence and comprehensive world understanding. However, in order to achieve human-like performance in real-world tasks, these models must be able to manage the interactive information acquired in continuous and diverse environments. Current LLMs primarily manage information through two memory mechanisms: contextual memory and compression-based parametric memory. While these mechanisms excel in short-term tasks, they are inadequate in supporting long-term autonomous learning and evolution.

\subsubsection{Textual Contextual Memory}

Textual contextual memory in models serves to retain and utilize current context information during a single inference call. It relies on key-value (KV) caches to store representations of all preceding tokens, facilitating better understanding and generation of task-relevant content. However, from a self-evolutionary perspective, this mechanism has several key limitations:

\begin{itemize}
\item \textbf{Temporality:} Stored contextual information is confined to the current task's scope, discarding previous states and sequence information upon completion of a single inference call.
\item \textbf{Lack of Long-Term Learning:} Transformer models possess only "working memory" during each call, lacking an inherent memory mechanism for retaining state information across calls, unlike Long Short-Term Memory (LSTM) networks \cite{hochreiter1997long}.
\item \textbf{Limited Knowledge Integration:} While the context window effectively utilizes current task information, it fails to accumulate and integrate knowledge across tasks and domains, which is crucial for continuous model evolution.
\item \textbf{Absence of Autonomous Learning Capability:} Current contextual memory mechanisms do not support autonomous pattern or rule discovery, limiting the model's ability to self-improve without explicit guidance.
\end{itemize}

\subsubsection{Compression-Based Parameter Memory}
The second mechanism is compression-based memory, which works by condensing world knowledge into the model's parameters, forming a kind of long-term memory \cite{brown2020fslearner}. This mechanism allows the model to retain crucial information over extended periods, but it comes with two significant drawbacks. 

\begin{itemize}
    \item \textbf{Inability to update in real-time:} Since the model’s parameters are fixed during the training process, the long-term memory cannot be easily updated once training is completed. This limitation poses challenges for personalization and adapting to dynamic environments, as the model cannot quickly learn new information or adjust its memory.
    
    \item \textbf{Difficulty in expressing individual data:} As a statistical model, the Transformer struggles to adequately represent individual data within its long-term memory. This often results in one of two outcomes: either the model fails to retain the individual data, or it overfits and forgets the previously stored world knowledge, leading to memory bias. The current approach to mitigating this issue involves incremental training with carefully balanced data proportions to incorporate individual data into the model. However, this process is inefficient and challenging to scale in large or dynamic data environments.
\end{itemize}

\subsection{Drawing Inspiration from Human Long-Term Memory}
\label{subsec:def_HLTM}

To better understand this, we can draw inspiration from the concept of human LTM, which provides a valuable framework for understanding how to achieve personalization.
%\subsubsection{Brief Review of LTM in Human Memory}
Existing neuroscience research indicates that personal memories generated through human interaction with the world are key factors in the formation of diverse and personalized behaviors. Current studies typically classify human memory into three main types: working memory, short-term memory, and long-term memory. Working memory and short-term memory mainly consist of temporary information related to the current task or scenario, which, if not processed and converted into long-term memory, will be quickly forgotten. Therefore, it can be considered that long-term memory serves as the critical data foundation for human personality formation.


To be more specific, human LTM refers to the capacity of the brain to store and retrieve information over extended periods, ranging from hours to decades \cite{McGaugh2000}. Unlike short-term memory, which holds information temporarily for immediate use, LTM is responsible for the preservation of knowledge and experiences that can influence our future behavior \cite{Squire2004, Sridhar2023}. This type of memory encompasses various subtypes, including episodic memory (personal experiences), semantic memory (general knowledge), and procedural memory (skills and habits)~\cite{Merlo2024}.

The formation of LTM involves several processes, including encoding, consolidation, and retrieval \cite{Straube2012}. Encoding refers to the initial acquisition of information, while consolidation is the process of stabilizing and integrating new information into existing memory networks \cite{Dudai2004}. Retrieval involves accessing and utilizing stored information when needed. These mechanisms are supported by neural processes in the brain, including the hippocampus and various cortical regions \cite{Squire2011}.

\subsubsection{LTM Enable Human Personalities in Various Aspects}

Human memory is a fundamental aspect of human cognition, a dynamic and multifaceted process that plays a critical role in shaping our existence~\cite{Schacter2007}. It is not merely a passive repository of past experiences but an active force that transcends direct experience to influence our survival, identity, and individual characteristics~\cite{Nairne2016}. 

The human memory system encompasses a wide variety of memories, and different types of memories serve different functions in human cognition ~\cite{Squire2011}. Of these, long-term memory needs to be singled out as the one that shapes our beliefs, values, and behaviors and contributes to the formation of our unique personality traits ~\cite{Madan2024, McAdams1996}.

Building on previous research, we recognize that long-term memory not only influences the formation of personal interests and habits but also plays a crucial role in the emergence of diverse needs\cite{sutin2023five}. Furthermore, long-term memory significantly impacts an individual's knowledge accumulation\cite{kenett2023thirst}, problem-solving abilities\cite{hambrick2003role}, social adaptability, and self-regulation\cite{zhao2011social}, leading to differentiated expressions of intelligence development and evolution. In social life, the social experiences and memories stored in long-term memory help individuals establish trust, facilitate knowledge and resource sharing, and ultimately foster collaboration and cooperation\cite{weldon1997collective}.

\begin{itemize}
    \item \textbf{Capability Growth.} The diverse capabilities of humans arise from long-term memory (LTM), which allows individuals to generalize and adapt their abilities to different contexts. LTM stores specific experiences while also abstracting principles from them. This enables us to extract relevant information to address various tasks. Neuroplasticity\cite{Fan-2023-NeuroAI}\cite{Sweatt2016}further supports this by restructuring neural connections based on experience, facilitating adjustments in behavior and abilities across situations.

    \item \textbf{Diverse Personality.} Long-term memory plays a pivotal role in shaping personal identity~\cite{Klein2012}. Our memories of past experiences, relationships, and achievements contribute to our self-concept and personal narrative~\cite{Greenberg2010}. By recalling and reflecting on these memories, we develop a consistent sense of who we are, including our values, preferences, and behaviors~\cite{Bauer2015}. For example, positive childhood experiences may foster a sense of confidence and optimism, while challenging experiences might influence resilience and adaptability.
    
    \item \textbf{Tailored Expertise.} HLTM also impacts our behavioral preferences and choices~\cite{Dolan2013,Kaushik2023}. Memories of past experiences help us make decisions by influencing our likes and dislikes. For instance, if someone has fond memories of a particular hobby, they are more likely to continue engaging in that activity~\cite{Rogers2020}. Similarly, negative experiences can lead to avoidance of certain situations or behaviors. This process of memory-based decision-making helps personalize our interactions with the environment and guide our daily choices~\cite{Biderman2021}.
\end{itemize}


\subsubsection{Human Long-Term Memory Utilization Mechanisms}
LTM is the basic resource in supporting human personalities, and the next question is how humans utilize LTM, which contains several key mechanisms, including:

\begin{itemize}
    \item \textbf{Memory Refinement.} The brain does not indiscriminately store and process all incoming data, but instead engages in a highly selective updating process\cite{Cowan1988}, encoding only the most salient and relevant information into Long-Term Memory (LTM). This intricate operation is governed by the interplay of reinforcement mechanisms and immediate encoding strategies, which work in tandem to prioritize the retention of significant experiences. Through this dynamic filtering, the brain ensures that the vast influx of sensory input is distilled into meaningful, durable memories, preserving only those elements that bear relevance to our ongoing cognitive framework and future behavior.
    \item \textbf{Continuously Updating.} Routine information is reinforced through repeated exposure and practice, with the hippocampus strengthening the connections between neurons (known as synaptic plasticity), making recall easier over time and solidifying the memory. On the other hand, when an experience is accompanied by strong emotions, such as during a sudden or significant event, the brain does not require repetition. In these cases, the amygdala works in concert with the hippocampus to enhance the encoding and consolidation of these emotionally charged memories\cite{richter2000amygdala} \cite{pare2003role} \cite{qasim2023neuronal}. This collaboration ensures that critical information is encoded instantly and retained more vividly. This dual approach—reinforcement for routine data and instant encoding for emotionally significant or survival-related information—provides the brain with a versatile and highly efficient learning system.
    \item \textbf{Efficient Utilization.} The human brain is designed for efficiency, making targeted updates to a limited number of neurons instead of extensive changes across the entire network. This selective updating allows for memory refinement based on relevance, minimizing cognitive load. Mechanisms like synaptic plasticity strengthen frequently used connections while less relevant pathways weaken over time. By focusing on essential neural connections, the brain retrieves information quickly and accurately without unnecessary strain. This efficiency enhances learning and optimizes memory storage, allowing the brain to function effectively in complex environments while conserving energy. 
\end{itemize}


\subsection{Can LTM Enable Model Personalization?}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{AILTM/figures/section_3/cde.png}
    \caption{The difference between human learning and growth versus artificial intelligence training and evolution. }
\end{figure}

In the previous section, we highlighted the significant role of LTM in human personalization, supported by a comprehensive mechanism for memory formation, updating, and utilization that ensures LTM serves personalization effectively. Considering that many aspects of model design and development draw inspiration from human cognitive and reasoning structures, such as the propagation mechanisms of neural networks is a classic example, if LTM can aid in human personalization, could it also be leveraged for model personalization? Our answer is definitely yes, and we discuss it from the following perspectives:

\begin{itemize}
    \item \textbf{From the Perspective of Data Accumulation:}
    Both models and humans interact extensively with their environments, providing foundational data for personalization processes. Unlike humans, AI models interact with their environments at much higher efficiency and can perform these interactions and iterations in purely virtual, digital environments. Therefore, with the design of appropriate Memory Refinement strategies, models should be able to accumulate LTM similarly to humans.

    \item \textbf{From the Perspective of Model Updates.} 
    AI excels in storing and recalling vast amounts of data, far surpassing human memory in scale. Neural networks manage this data through distributed parameters, handling inputs across various domains. However, this storage is rigid, lacking the flexibility for real-time updates without retraining. In contrast, human memory is adaptive, integrating new information quickly while discarding outdated details through a process known as adaptive forgetting. This flexibility helps humans avoid cognitive overload and focus on what's relevant at any given moment. To match this capability, AI systems would need dynamic updating mechanisms that allow them to discard outdated knowledge without full retraining.

    \item \textbf{From the Perspective of LTM Utilization.}
    The current advanced LLM memory mechanisms, represented by in-context memory and parametric memory, enable the storage and utilization of information with the advantage of non-forgetfulness. Additionally, AI can incorporate mechanisms for instant memory updates when encountering significant new data, which is especially useful in dynamic environments. This provides a certain advantage over human memory utilization. However, these memory utilization methods still face significant challenges in managing dynamically accumulated LTM, making it difficult to achieve efficient memory utilization like humans, particularly in the aspect of memory updating.
\end{itemize}

In summary, the success of human LTM offers a valuable blueprint for achieving model personalization. We believe that the technical path is feasible. While human memory excels in contextual integration, flexibility, and real-time updating, AI shines in managing large datasets and recognizing patterns at scale. To harness the strengths of human memory, AI must integrate flexibility with scale, prioritization, and efficient updating. This hybrid approach could produce AI models that are more personalized, responsive, and context-aware, closely mimicking human cognitive complexity and adaptability.

\subsection{Definition of LTM for Model Personalization}
Before discussing how to construct LTM and utilize LTM for model personalization, we first give the definition and clarify the importance of model LTM in this subsection.

\textbf{Definition: Model long-term memory refers to continuously-updated personal data, which can be collected, refined, and utilized for support model personalization.}

Just as humans use LTM to shape their behaviors and identities, AI systems can leverage similar mechanisms to customize their responses and actions based on personal data. This "personal" aspect extends beyond individual users to include organizations and specific domains, allowing models to adapt their responses and behaviors based on a wider array of user-specific contexts and requirements. This forms the foundation for creating personalized models that go beyond generalized knowledge. As discussed in Section \ref{subsec:def_HLTM}, human LTM refers to the brain's ability to store and retrieve information over extended periods, encompassing the knowledge and experiences that shape our behaviors, identity, and interactions \cite{Sridhar2023}. Similarly, LTM refers to the data, knowledge, and experiences that shape an AI model's behavior over time.


LTM can be understood as a vast and complex repository of refined knowledge, shaped over time by a group of independent yet harmoniously interacting agents—agents that resemble the cortical columns of the brain. Each agent, functioning as an autonomous unit, is capable of learning, refining, and storing a comprehensive model of its own corner of the world. However, these agents do not operate in isolation; they contribute their insights to the broader collective of the LTM, creating a shared knowledge base that supports deeply personalized interactions.

Unlike traditional, static data storage systems, the LTM is a dynamic and adaptive entity. It constantly evolves, updated by agents in response to environmental changes and absorbing new individual inputs. This ongoing evolution enables the system to adapt with remarkable fluidity, refining its structure and responses to meet the ever-changing needs and contexts of the individuals it interacts with.

This distributed memory framework, akin to a network of independently functioning minds, allows insights from various independent learning processes to be synthesized. Just as a society gathers to form a more cohesive understanding, this collective intelligence enables the system to not only accumulate knowledge but also synthesize it in a way that better aligns with the complexity and subtleties of user needs. The result is a more nuanced and comprehensive understanding, enabling the system to respond to individual needs with a sophistication that reflects the intricacy of those needs. In this sense, LTM transcends mere data storage—it becomes an adaptive, ever-evolving cognitive organism, continuously refining itself in response to the environment, much like the human cognition it seeks to emulate.

\subsection{Importance of LTM for Models} \subsubsection{LTM for Model Personalization} LTM is pivotal for model personalization, as it enables models to tailor interactions based on a deep understanding of individual individuals. By recalling past interactions, recognizing preferences, and adapting to contextual changes over time, LTM allows AI systems to generalize from historical data and provide adaptive responses in novel situations. This capability is rooted in the encoding of information within the neural network’s weights and parameters, which is crucial for supporting personalized interactions and continuous learning \cite{Zhong2024}.

The distributed and dynamic nature of LTM allows AI systems to refine interactions based on historical data, individual preferences, and context \cite{Du2024}. Ultimately, integrating LTM into AI models represents a significant step toward advanced, human-like personalization. By retaining and utilizing long-term data, LTM lays the foundation for personalized, context-aware interactions that evolve over time. As AI continues to advance, the development of LTM will be key to creating systems that not only understand but also anticipate and adapt to the unique needs of individuals, providing a truly personalized experience.

\subsubsection{LTM for the Self-Evolution of Personalized Model}
The self-evolution capability of models is a highly promising direction for the development and application of AI technologies. Just as human intelligence relies on personal interactions and feedback from real-world environments, the LTM data accumulated by models during interactions also contributes to model personalization, providing the most crucial data support for self-evolution. While there are also some differences:

Unlike human evolution, LTM-driven model evolution is not limited to real-world interactions. On the one hand, models can interact with the physical environment like humans and receive direct feedback, which, after processing, leads to enhanced capabilities. This is also a key area of research in embodied AI. On the other hand, models can interact and accumulate LTM data in virtual environments, which offers lower costs and higher efficiency compared to real-world interactions, thus enabling more effective capability enhancement.

In contrast to the existing approaches that directly store interaction history and reflections, refined LTM data can provide higher-quality data support for model self-evolution, further accelerating the efficiency and effectiveness of the model's evolution. This provides more effective support for improving the capabilities and rapid application of LLMs-powered agents.

After clarifying the importance of LTM for AI models, especially for model personalization, we will focus on discussing the following two questions: 1) how to construct LTM? (Section \ref{subsec:how_to_LTM}) 2) How can LTM be used to achieve model personalization in AI Self-Evolution? (Section \ref{subsec:how_to_integrate}). 



% Human memory offers a sophisticated model for inspiring AI, especially in the design of memory systems that enhance learning and adaptation. By emulating how the brain processes and prioritizes information, AI systems can better handle dynamic inputs and focus on relevant data.

% In AI, human memory mechanisms can be adapted to boost model performance. Reinforcement learning, for example, enables AI to refine its actions based on environmental feedback, similar to how neural pathways are strengthened in the brain. Additionally, AI can incorporate mechanisms for instant memory updates when encountering significant new data, which is especially useful in dynamic environments. 

% AI excels in storing and recalling vast amounts of data, far surpassing human memory in scale. Neural networks manage this data through distributed parameters, handling inputs across various domains. However, this storage is rigid, lacking the flexibility for real-time updates without retraining. In contrast, human memory is adaptive, integrating new information quickly while discarding outdated details through a process known as adaptive forgetting. This flexibility helps humans avoid cognitive overload and focus on what's relevant at any given moment. To match this capability, AI systems would need dynamic updating mechanisms that allow them to discard outdated knowledge without full retraining.

% A notable aspect of human memory is its ability to integrate information from various contexts, creating a rich and nuanced understanding. Humans combine sensory input, emotional experiences, and prior knowledge to build a coherent view of new information. AI models, like transformers with self-attention mechanisms, aim to mimic this by analyzing sequential data and identifying patterns across contexts~\cite{vaswani_attention_2017}. However, current models still struggle with maintaining contextual nuance, especially when switching between different domains or tasks. Enhancing attention mechanisms and improving context-awareness could help AI better replicate the integrative abilities of human memory.

% AI has advanced in learning from large datasets, but its compression-based memory mechanism presents challenges. Once trained, the model’s parameters are fixed, so it can't update its memory in real-time. This contrasts sharply with human memory, which continuously updates and retrieves context-specific information. Humans can quickly adapt to new information, whereas AI requires incremental retraining for updates, leading to inefficiencies. Additionally, AI struggles with expressing individual data without bias or overfitting. Balancing global knowledge with personalized data remains a challenge in AI's long-term memory \cite{brown2020fslearner}.

% In summary, human memory offers a valuable blueprint for creating more adaptive and efficient AI systems. While human memory excels in contextual integration, flexibility, and real-time updating, AI shines in managing large datasets and recognizing patterns at scale. To harness the strengths of human memory, AI must integrate flexibility with scale, prioritization, and efficient updating. This hybrid approach could produce AI models that are more personalized, responsive, and context-aware, closely mimicking human cognitive complexity and adaptability.


% Long-term memory is central to the concept of model personalization because it allows AI systems to store, retrieve, and adapt based on a user’s individual preferences, behaviors, and experiences over time. 

==> new_sections/backup_04.tex <==
 
\section{LTM for Model Personalization}
% -------- start story line------------------------
%
%本文的重点不是LLM的记忆机制；但是要对模型个性化，所以需要了解模型对于记忆的工作机制
%LLM有2种记忆机制：
%1，context window，这个机制对于模型个性化有一定的体现；缺点是这种方式不是显式的存储机制，仅依赖KV缓存将之前所有token的表示存储在一个列表中。 这种设计意味着，一旦query在一次调用中完成，Transformer就不会在后续调用中保留或回忆任何先前的状态或序列， 因此，Transformer在每次调用期间只具有上下文中的工作记忆，而不是诸如长短期记忆(LSTM)等固有记忆机制。
%2，通过压缩，将世界知识压缩为参数。这是模型的长期记忆机制，缺点是
%   a，无法实时更新，
%   b，因为是个统计模型，个体的数据进入模型很难被显著的表达。表现的形式是，个体的数据进入模型，要么记不住，要么过拟合忘记世界知识，目前做法是通过精细的数据配比进行增量训练，效率很低；

% 不同区域，不存在一个超级llm，进入模型之后的，都是ltm==模型的个性化

%长期意味序列化，分区存储，一种基础结构解析和存储所有？以一种唯一的形态存储数据可行吗?

%模型是对数据的压缩，从这个角度来说，如果把现在的llm看做是一个 5000 年寿命，70 亿体细胞的单一个体的话，对这个给他而言，每个单独细胞贡献的数据是构成了这个，以此往下推论，个性化的模型，就是训练得到个这个个性化模型所需要的数据。

%如前文模型个性化讨论的，参考生命进化和计算机系统演变的历程，不太可能存在一个超级的单一个体，这个过程在生命的进化（举例）pc,移动手机一次次的上演，而模型很有可能也会经历这样的演话，从超级模型很可能变成个性化模型

%对于超级模型而言，长期记忆是训练这个超级模型的所有数据，即Compression-Based Memory，本文的重点在论述模型个性化，在基础模型之上，用于训练模型个性化的数据，就是长期记忆。
% 在我们的观点 zhong，模型的能力会不断的上涨，所以这些记忆和插头一样，应该允许他插拔这不同的基础模型之上，然后通过seection6的方法，让这些数据被体现出来。




% 裸数据是长期记忆吗？是的，我们强调，所有对于模型训练有用的数据，都是长期记忆，即便现在还没有合适的处理方法，这些数据应该被优先储存下来。
%特别强调，零碎的散落的 raw data，被汇聚起来后，就从短期记忆变成了长期记忆，长期记忆顾名思义，意味着更长的时间和空间维度，序列化的数据更能体现价值
% 长期记忆的形态？% 长期记忆有包括哪些数据？以什么样的形式存在？
% 上文中，把llm 类比为单一个体，把 context window 类比为 工作记忆，把 模型权重类比为 这个单一个体的长期记忆，那么，对于模型的个性化，长期记忆的存储形式也是以参数化为唯一性形态吗？
% 不是，还是类比人类脑区，不同的输入形态有不同和区域，比如视觉（枕叶，听觉，颞叶）等，这些原始的输入在不同的区域处理后，输入的数据被参数化有存储在各自的位置；同时，这些数据也被海马体加工后，

% B. 说明Memory为什么无法替代AILTM（解释为啥需要refine）
% a. memory是对客观世界的直接观察和记录，存在大量冗余信息，这些信息对于模型个性化没有帮助
% b. memory是离散的，但是AILTM是互相关联的（类比HLTM需要大脑处理后才是LTM），这些关联是服务推理的必要因素
% 			c. ... (可补充)

% -------------end story line  -------------------

% Human LTM demonstrates that how accumulated memories and dynamic updates help us navigate complex environments. This serves as a key inspiration for designing similar mechanisms in AI models. Next, we introduce the concept of model LTM, which is not just a memory store, but a system of adaptable parameters that can evolve over time to support personalized experiences.

% This section reviews the memory mechanisms inherent in large language models (LLMs). Following this, a formal definition of Long-Term Memory (LTM) is proposed, alongside a discussion of its significance in the context of AI-driven personalization. Model LTM is further distinguished from raw data storage, highlighting its unique role. Lastly, we explore the critical importance of LTM in advancing model personalization.

%开头提出我们这章重点介绍model LTM，首先回顾LLM中的记忆机制，然后提出长期记忆的正式定义，并将其与raw data进行区分。最后探讨LTM在推动模型个性化中的关键作用。
Human LTM demonstrates how accumulated memories and dynamic updates help us navigate complex environments, serving as a key inspiration for designing similar mechanisms in AI models. Building on this inspiration, we introduce the concept of model LTM, which extends beyond a simple memory store to become a system of adaptable parameters that evolve over time, supporting personalized experiences.

In this context, we first review the memory mechanisms inherent in large language models and then propose a formal definition of Long-Term Memory (LTM). We discuss its significance in AI-driven personalization, distinguishing model LTM from raw data storage to highlight its unique role. Finally, we explore the critical importance of LTM in advancing model personalization.

% 在讨论开始之前，先讨论一下目前 llm 的2 种记忆机制，
\subsection{Current Memory Mechanisms of LLMs}

LLMs, such as GPT-4 and Gemini, exhibit advanced intelligence and a comprehensive understanding of the world. However, to effectively manage specific real-world situations, these models must be capable of processing and storing information obtained through their interactions with various environments. This is facilitated by distinct memory mechanisms, primarily the In-Context Memory and Compression-Based Memory.

\subsubsection{In-Context Memory}
The In-Context Memory mechanism plays a role in model memorization by retaining and utilizing the current context information during a single inference call. It relies on a Key-Value (KV) cache to store the representations of all preceding tokens in a list, allowing the model to better understand and generate content relevant to the ongoing task. However, this mechanism is not an explicit storage method; the stored context information is limited to the scope of the current task. Once a query is completed in a single inference call, the Transformer model discards the previous state and sequence information, meaning it does not retain or recall any prior context in subsequent inferences. Consequently, the Transformer only possesses "working memory" during each call—temporary memory from the current context—rather than an inherent memory mechanism like Long Short-Term Memory (LSTM)~\cite{hochreiter1997long} that can retain state information across calls. While the Context Window effectively leverages context information for the current task, its memory is transient and limited, providing no lasting memory support for the model.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{AILTM/figures/section_4/LTMvsLLMMemory.png}
    \caption{Comparison of LLM Memory and Long-Term Memory}
    \label{fig:ltm_vs_llm_memory}
\end{figure}

\subsubsection{Compression-Based Memory}
The second mechanism is compression-based memory, which works by condensing world knowledge into the model's parameters, forming a kind of long-term memory \cite{brown2020fslearner}. This mechanism allows the model to retain crucial information over extended periods, but it comes with two significant drawbacks. First, Inability to update in real-time: Since the model’s parameters are fixed during the training process, the long-term memory cannot be easily updated once training is completed. This limitation poses challenges for personalization and adapting to dynamic environments, as the model cannot quickly learn new information or adjust its memory. Second, Difficulty in expressing individual data: As a statistical model, the Transformer struggles to adequately represent individual data within its long-term memory. This often results in one of two outcomes: either the model fails to retain the individual data, or it overfits and forgets the previously stored world knowledge, leading to memory bias. The current approach to mitigating this issue involves incremental training with carefully balanced data proportions to incorporate individual data into the model. However, this process is inefficient and challenging to scale in large or dynamic data environments.

\subsection{Leveraging Human Memory Mechanisms}

Human memory offers a sophisticated model for inspiring AI, especially in in the design of memory systems that enhance learning and adaptation. By emulating how the brain processes and prioritizes information, AI systems can better handle dynamic inputs and focus on relevant data.

One of the most remarkable features of human memory is its efficiency in filtering information. The brain does not process every piece of incoming data equally; instead, it selectively updates, encoding only the most important and relevant information into long-term memory. This process is governed by both reinforcement and instant encoding mechanisms. Routine information is reinforced through repeated exposure and practice, with the hippocampus strengthening the connections between neurons (known as synaptic plasticity), making recall easier over time and solidifying the memory.On the other hand, when an experience is accompanied by strong emotions, such as during a sudden or significant event, the brain does not require repetition. In these cases, the amygdala works in concert with the hippocampus to enhance the encoding and consolidation of these emotionally charged memories\cite{richter2000amygdala} \cite{pare2003role} \cite{qasim2023neuronal} . This collaboration ensures that critical information is encoded instantly and retained more vividly.This dual approach—reinforcement for routine data and instant encoding for emotionally significant or survival-related information—provides the brain with a versatile and highly efficient learning system.

In AI, human memory mechanisms can be adapted to boost model performance. Reinforcement learning, for example, enables AI to refine its actions based on environmental feedback, similar to how neural pathways are strengthened in the brain. Additionally, AI can incorporate mechanisms for instant memory updates when encountering significant new data, which is especially useful in dynamic environments. 

AI excels in storing and recalling vast amounts of data, far surpassing human memory in scale. Neural networks manage this data through distributed parameters, handling inputs across various domains. However, this storage is rigid, lacking the flexibility for real-time updates without retraining. In contrast, human memory is adaptive, integrating new information quickly while discarding outdated details through a process known as adaptive forgetting. This flexibility helps humans avoid cognitive overload and focus on what's relevant at any given moment. To match this capability, AI systems would need dynamic updating mechanisms that allow them to discard outdated knowledge without full retraining.

\MY{we talked about human memory excels in filtering information in previous paragraphs; maybe use bullet list or textbf to make the CAPABILITY helpful in humans and machines as clues? i.e. \paragraph{Information filtering capability.} and then elaborate on humans and machines.}
A notable aspect of human memory is its ability to integrate information from various contexts, creating a rich and nuanced understanding. Humans combine sensory input, emotional experiences, and prior knowledge to build a coherent view of new information. AI models, like transformers with self-attention mechanisms, aim to mimic this by analyzing sequential data and identifying patterns across contexts~\cite{vaswani_attention_2017}. However, current models still struggle with maintaining contextual nuance, especially when switching between different domains or tasks. Enhancing attention mechanisms and improving context-awareness could help AI better replicate the integrative abilities of human memory.

AI has advanced in learning from large datasets, but its compression-based memory mechanism presents challenges. Once trained, the model’s parameters are fixed, so it can't update its memory in real-time. This contrasts sharply with human memory, which continuously updates and retrieves context-specific information. Humans can quickly adapt to new information, whereas AI requires incremental retraining for updates, leading to inefficiencies. Additionally, AI struggles with expressing individual data without bias or overfitting. Balancing global knowledge with personalized data remains a challenge in AI's long-term memory \cite{brown2020fslearner}.

In summary, human memory offers a valuable blueprint for creating more adaptive and efficient AI systems. While human memory excels in contextual integration, flexibility, and real-time updating, AI shines in managing large datasets and recognizing patterns at scale. To harness the strengths of human memory, AI must integrate flexibility with scale, prioritization, and efficient updating. This hybrid approach could produce AI models that are more personalized, responsive, and context-aware, closely mimicking human cognitive complexity and adaptability.

\subsection{Definition of Long-Term Memory in Model Personalization}

Long-term memory is central to the concept of model personalization because it allows AI systems to store, retrieve, and adapt based on a user’s individual preferences, behaviors, and experiences over time. Just as humans use long-term memory to shape their behaviors and identities, AI systems can leverage similar mechanisms to customize their responses and actions for each individual user. This forms the foundation for creating personalized models that go beyond generalized knowledge.


As discussed in \ref{subsec:def_HLTM}, human LTM refers to the brain's ability to store and retrieve information over extended periods, encompassing the knowledge and experiences that shape our behaviors, identity, and interactions \cite{Sridhar2023}. Similarly, LTM refers to the data, knowledge, and experiences that shape an AI model's behavior over time.

We propose the following definition for Long-Term Memory (LTM) \MY{for model personalization}: 
LTM is a collection of all refined data and information accumulated and retained over time by multiple independent but collaboratively functioning agents, analogous to cortical columns in the brain, to support personalized interactions. Each agent can independently learn and store a complete world model, integrating its experiences into the LTM. Unlike raw data storage, LTM is dynamically updated by these agents based on environmental changes and user input, allowing for continuous adaptation and personalization. This distributed memory structure enables the system to consolidate the results of multiple independent learning processes, leading to a more comprehensive understanding and response to user needs.
\MY{I would put current 4.3 / 4.4 as a new section to highlight the focus of this work and match the research questions raised at the beginning; if 2 stands alone, then section 3 and former part of section 4 can stay in one section: Human and Machine Memory Structure}
%it is the aggregation of all refined data and information an AI model retains over time to support personalized interactions. To better illustrate this definition, we distinguish LTM from raw data storage. Unlike raw data, LTM dynamically updates according to environmental changes and user inputs, allowing for continuous adaptation and personalization.



%\subsubsection{AILTM Vs. AI Short Term Memory(AISTM)}

%Short Term Memory (STM) is designed for specific, immediate tasks. It focuses on retaining information relevant to the current context or session. AISTM is often implemented using a context window, which temporarily holds data needed for the task at hand, such as recent conversation history or the current state of a process.
%In contrast, Long-Term Memory (LTM) is comprehensive and accumulates knowledge from various sources, allowing the AI to provide more contextual and relevant responses based on historical data.
%The relationship between LTM and STM is complementary. While AISTM provides the AI with the ability to handle immediate, context-specific tasks efficiently, AILTM ensures that the AI can draw on a broader, more comprehensive knowledge base to inform its actions and decisions. AILTM can be implemented using various methods, including databases, knowledge graphs, and other long-term storage solutions, ensuring that the AI retains valuable information over extended periods.


% \subsubsection{LTM and Raw Data}

% Raw Data Memory represents the comprehensive collection of all unprocessed data that a model receives through interactions with the external environment or during the training process. This data includes a wide range of observations and records, which may contain both valuable patterns and large amounts of redundant or irrelevant information. While Raw Data Memory forms the foundational layer for the model's memory and cognition, it requires further processing to be effectively used for personalization or efficient task execution.

% LTM refines and structures this raw data, making it usable by the model. This process enhances the model's ability to deliver personalized responses and recommendations. While Raw Data Memory captures direct observations that may result in redundancy and clutter, LTM organizes this data into a structured memory, enabling the model to recognize patterns, remember preferences, and provide adaptive responses.

% For instance, in an AI medical scenario, Raw Data Memory might capture basic patient information, such as demographic details, current symptoms, and immediate diagnoses. However, Raw Data Memory alone would struggle to effectively manage and integrate a patient’s comprehensive health history into a cohesive understanding of their condition.

% In contrast, LTM refines and organizes this raw patient data into an interconnected structure, allowing the AI model to draw meaningful inferences from the patient’s entire medical history. This supports advanced reasoning and personalized healthcare solutions. LTM would not only retain a patient’s ongoing medication regimen but also relate it to their historical response to similar treatments, recognize patterns in evolving symptoms, and adapt recommendations accordingly. This refined memory enables the AI model to facilitate advanced reasoning and personalized healthcare that evolves over time, delivering deeply individualized care.

% In conclusion, while Raw Data Memory provides a foundation for immediate context management, LTM is indispensable for achieving the deep, sustained personalization necessary for AI systems to remain relevant and effective. This allows AI to deliver richer, more personalized experiences that continuously improve and adapt to real-world complexities.

\subsection{Importance of LTM in Model Personalization}
Long-Term Memory (LTM) is pivotal for AI personalization, as it enables models to tailor interactions based on a deep understanding of individual users. By recalling past interactions, recognizing preferences, and adapting to contextual changes over time, LTM allows AI systems to generalize from historical data and provide adaptive responses in novel situations. This capability is rooted in the encoding of information within the neural network’s weights and parameters, which is crucial for supporting personalized interactions and continuous learning \cite{Zhong2024}.

The distributed and dynamic nature of LTM allows AI systems to refine interactions based on historical data, user preferences, and context \cite{Du2024}. Ultimately, integrating LTM into AI models represents a significant step toward advanced, human-like personalization. By retaining and utilizing long-term data, LTM lays the foundation for personalized, context-aware interactions that evolve over time. As AI continues to advance, the development of LTM will be key to creating systems that not only understand but also anticipate and adapt to the unique needs of users, providing a truly personalized experience.

==> new_sections/backup_06.tex <==
\section{How to Achieve Model Personalization with LTM?}
% -------- start story line------------------------

%此章回答引言中的第二个问题：如何利用长期记忆数据实现模型个性化。介绍两种实现方式：
% * discussion: multi-agent
%1. RAG+Muti-agents方法：通过这种方法构建长期记忆，并分析其存在的局限性，及行业前沿的最新进展。引入agent和多agent系统，帮助构建个性化长期记忆。然而，这种方法的局限在于仅能记住数据而无法学习数据中的行为模式。LLM提供分析规划能力的前额叶的LLM仍然是世界模型，不是个性化的。
%最新的方法是让agent在环境中自我进化，成为内化个性化的记忆驱动型agent。（介绍和清华的muti-agent自进化框架，在这个部分体现）

%2. 数据驱动的个性化训练：通过继续预训练、SFT、PEFT或ICL等方式，将个体数据直接训练进模型。（xav）

% -------------end story line  -------------------

After acquiring the high-quality LTM data, the next challenge we face is how to use it to achieve model personalization. There are several key challenges need to be addressed in the process of using LTM data to maximize its effectiveness and efficiency, including:

\begin{itemize}
    \item \textbf{Adapting to Continuously Updated LTM Data}. As user LTM data is continuously accumulated, the model must balance learning new information while retaining previously acquired knowledge. Traditional models often assume stable data distributions, but in real scenarios, new LTM data may significantly diverge from earlier patterns, leading to risks like overfitting or catastrophic forgetting. Efficiently handling these shifts is critical to adapt to the dynamic LTM data.
    \item \textbf{Real-Time Learning and Efficient Feedback Integration}. Due to the LTM data being accumulated dynamically, models must quickly adapt to real-time changes in user behavior. Rapid integration of new data is vital for applications such as intelligent assistants, where seamless user interaction is key. Besides, user feedback, both implicit (e.g., clicks or time spent) and explicit, should be taken into consideration when refining the foundation model. % While implicit feedback is easier to gather, explicit feedback offers more reliable insights. 
    Incorporating both types of feedback in real-time enables the model to continuously improve and align with individual user needs.% Effective integration of this feedback ensures the system remains responsive and relevant.
    \item \textbf{Handling Data Sparsity and User Diversity}. Data sparsity is a common issue in continuously updated LTM systems, especially for users with limited interaction history or sporadic activity, making it difficult to train personalized models. Furthermore, User diversity adds further complexity, requiring the model to adapt to individual patterns while still generalizing effectively across diverse user groups.
\end{itemize}

In the following subsections, we will review existing efforts that can be adopted to solve these challenges and summarize their weaknesses. Note that LLMs have become the most powerful AI models, the model personalization discussion will also focus on using LTM combined with LLMs.


% \subsection{Challenges of Continuously Updated LTM}
% Continuously updating long-term memory (LTM) models presents several technical challenges, including managing vast amounts of evolving user data, adapting to shifting data patterns, and ensuring accuracy over time.

% \subsubsection{Handling Data Sparsity and User Diversity in Continuous Updates}

% Data sparsity is a common issue in continuously updated LTM systems, especially for users with limited interaction history or sporadic activity. Personalized models often work with smaller and evolving datasets, making it difficult to generate precise predictions, particularly in the early stages.

% User diversity adds further complexity. Each user exhibits unique behaviors and preferences, requiring the model to adapt to individual patterns while still generalizing effectively across diverse user groups. Achieving a balance between personalization and generalization is crucial for long-term success.

% \subsubsection{Real-Time Learning and Efficient Feedback Integration}

% In continuously updated LTM systems, models must quickly adapt to real-time changes in user behavior. Rapid integration of new data is vital for applications such as intelligent assistants, where seamless user interaction is key. To achieve this, models need efficient knowledge updates without full retraining, which is resource-intensive. Low-latency processing and incremental updates are essential for maintaining timely and accurate responses.

% User feedback, both implicit (e.g., clicks or time spent) and explicit, is crucial for refining the model. While implicit feedback is easier to gather, explicit feedback offers more reliable insights. Incorporating both types of feedback in real time enables the model to continuously improve and align with individual user needs. Effective integration of this feedback ensures the system remains responsive and relevant.

% \subsubsection{Adapting to Dynamic Data Patterns}

% As user data continuously evolves, the model must balance learning new information while retaining previously acquired knowledge. Traditional models often assume stable data distributions, but in continuously updated systems, new data may significantly diverge from earlier patterns, leading to risks like overfitting or catastrophic forgetting. Efficiently handling these shifts in data distribution is critical, allowing old and new information to coexist without incurring high computational costs.

\subsection{Incorporating LTM as Outside Knowledge Bases}
%Integration LTM with Retrieval-Augmented Generation and In-Context Learning}

Since LTM is generated during interactions and may be refined with preprocessing, which is continuously updated, an intuitive strategy of utilization is to keep it independent from the foundation model, serving as an outside knowledge base to assist with reasoning and inference. While taking Transformer-based LLMs as an example, their structure inherently does not retain or recall any previous state or sequence, which limits the model's ability to carry LTM information but only short-term ``working memory'' for the current context window. 
So extra efforts should be made to address this limitation in utilizing LTM as outside knowledge bases for LLMs.

The most popular strategy in using an outside knowledge base for LLMs is Retrieval-Augmented Generation (RAG) with In-Context Learning (ICL), which can be adapted to utilize LTM data too. ICL mimics working memory, processing short-term information. Meanwhile, RAG, serving as an external database, acts as a module for LTM.


% As previously discussed, LLMs inherently lack an explicit memory mechanism. These models rely on key-value (KV) caching to store token representations within a limited context window during a single query, meaning that once the query is complete, the model does not retain or recall any previous state or sequence. This design limits the model’s ability to carry information across multiple interactions, giving it only short-term “working memory” for the current context window, unlike memory-rich models like Long Short-Term Memory (LSTM) networks, which can maintain information over extended sequences.

% To address this limitation, Retrieval-Augmented Generation (RAG) models have emerged as a popular approach to provide LLMs with external memory storage. 
% In the RAG+ paradigm, the LLM functions similarly to the human brain's prefrontal cortex, responsible for decision-making and planning, while ICL mimics working memory, processing short-term information. Meanwhile, RAG, serving as an external database, acts as a module for long-term memory.

As a comparison, the LLM's ICL ability to plan and reason improves as model size and capabilities grow, approaching—if not exceeding—the capacity of the human prefrontal cortex in specific domains. Human working memory is limited to a span of around 7±2 items, whereas modern LLMs, with increasingly large context windows (ranging from 4K to 1M tokens or more), can hold significantly more information. RAG, as an external storage mechanism, provides the potential for storing and retrieving an unlimited amount of information, which seemingly addresses the limitation of human memory by offering three analogous stages: encoding, storage, and generation.


\subsubsection{Advances in Memory Encoding, Storage, and Retrieval}

In this section, we first review existing efforts made in memory encoding, storage, and retrieval with RAG and ICL, which are necessary modules to utilize LTM to achieve model personalization. Although there are several challenges in distinct steps, techniques like adaptive memory pruning, more efficient indexing systems, and context-aware retrieval algorithms could help mitigate some of these issues. Additionally, integrating reinforcement learning-based feedback mechanisms could enable more selective memory encoding, allowing LLMs to prioritize important data and improve long-term retrieval accuracy.

% In light of the challenges faced in encoding, storage, and retrieval within LLM-based memory architectures, the latest advancements in retrieval-augmented generation (RAG) and in-context learning (ICL) aim to address these issues by drawing closer analogies to human memory processes. In this section, we will explore how RAG and ICL paradigms are evolving to mimic the three core stages of human memory: encoding, storage, and retrieval, while addressing the limitations outlined earlier.


\textbf{Encoding:} One of the most critical shortcomings of current LLM architectures is the indiscriminate nature of data encoding. Unlike human memory, which selects relevant information for long-term retention based on salience and context, LLMs encode vast amounts of information without prioritization, leading to bloated and inefficient memory systems. Recent advancements in RAG-based systems have focused on introducing mechanisms for selective encoding, similar to human memory. Models like MuRAG \cite{murag2022} and RA-CM3 \cite{racm322}, for instance, are integrating multimodal data (images, text) with refined hierarchical indexing systems. This approach mirrors how humans encode experiences from different sensory inputs, allowing the system to distinguish between relevant and irrelevant information, ensuring that only the most contextually pertinent data is encoded into memory. Additionally, recent techniques such as UPRISE \cite{uprise2023} offer promising methods to enhance memory encoding by constructing a pool of context-aware prompts, selectively retrieving relevant templates for different tasks. This dynamic process parallels how humans draw on past experiences when encoding new information, improving the efficiency and selectivity of memory formation.

\textbf{Storage:} While RAG architectures allow for unlimited data storage, they still struggle with consolidation, organization, and fragmentation of memories, which become more difficult to retrieve as the memory system grows. In contrast, human brains consolidate memories during rest periods, integrating and organizing information in a way that strengthens important memories while letting others fade. To address this, recent studies haved developed more structured storage systems, such as RAPTOR \cite{raptor2024} and MEMWALKER \cite{memwalker2023}, which take a step towards improving the hierarchical organization of stored information. These models introduce a tree-like structure that clusters and summarizes data recursively, creating a more structured memory space that allows for efficient retrieval of information across different levels of abstraction.
    
In addition, emerging models like $\text{Memory}^3$ \cite{Memory³} propose integrating explicit memory modules that manage knowledge as key-value pairs in external non-volatile storage, emulating how the human brain efficiently consolidates and accesses memories based on relevance and frequency of recall. Techniques like compressive memory, seen in Beyond Retrieval: Embracing Compressive Memory \cite{chen2024compressimpressunleashingpotential} , explore how to compress and store interactions while retaining the core elements of past experiences, thus reducing redundancy and improving access to the most relevant parts of memory during retrieval.

\textbf{Retrieval:} The retrieval process is where the largest divergence between human and LLM-based memory systems occurs. While humans rely on associative and context-driven recall, current LLM retrieval relies heavily on probabilistic token generation, often resulting in the retrieval of incomplete or irrelevant information. Recent work has shifted toward improving retrieval systems by introducing hybrid search techniques that blend traditional keyword-based search with more advanced semantic retrieval systems. For instance, Blended RAG \cite{blendedrag2024} and Hybrid Search \cite{hybridsearch2024} combine BM25 with dense vector embeddings to improve both the relevance and context-awareness of retrieved information. Moreover, methods like FiD emphasize the need for creating more sophisticated queries that better match the intent and structure of the memory database, drawing parallels to how humans refine their recall based on the specific context of a query.
    
Besides, post-retrieval mechanisms such as re-ranking and self-reflection, as seen in models like Self-RAG and Re2G[todo], aim to refine the retrieved information to align more closely with the user’s query. These systems not only filter out irrelevant content but also prioritize the most contextually appropriate responses, echoing how human memory retrieval is shaped by the relevance and importance of past experiences to the current situation.


To summarize, the RAG and ICL strategies do not require updating the foundation model’s parameters, allowing for efficient integration and updating of LTM data, which makes it possible to support real-time, efficient LTM management and utilization. The foundation model can achieve personalization with distinct LTM data through this strategy. However, despite improvements in memory encoding and retrieval, there is still a fundamental disconnect between the deep, associative nature of human memory and the more surface-level pattern recognition performed by LLMs. New models like MemoCRS and COMEDY[todo] represent initial attempts to bridge this gap by integrating deeper, long-term contextual memory into conversational AI, but much work remains in improving the depth and dynamism of memory representation.


%In conclusion, while the current trajectory of research is moving toward more human-like memory systems, achieving a truly seamless integration between LLM architectures and human memory processes will require continued innovation in dynamic memory management, context-aware retrieval, and more selective, adaptive encoding mechanisms. By drawing more directly on the principles of human memory—such as selective encoding, memory consolidation, and associative retrieval—future architectures could achieve a more efficient, scalable, and human-like memory model.

\subsubsection{Utilizing LTM with RAG-based Multi-Agents}

Except for the primary encoding, storage, and retrieval studies about how to utilize LTM in specific LLMs, we propose that LTM can also be adopted by using RAG-based multi-agent systems to achieve model personalization. Several interconnected strategies can be employed to create a cohesive and efficient memory framework that mimics human cognition, including 1) dynamic memory storage, 2) context-based retrieval, 3) memory consolidation, and 4) self-reflection, all within a multi-agent framework. In this framework, different agents can understand LTM patterns of user behavior and improve their decision-making and action planning, and we will introduce them one by one. Note that each module can be implemented by a single LLM-powered agent.

\textbf{1) Dynamic Memory Storage} is a key component in improving long-term memory is the dynamic management of stored information. Instead of passively accumulating data, memory systems must prioritize the retention of relevant information. This involves continuously updating the memory bank based on interaction context, user preferences, and relevance to the task. By applying a vectorized storage system, memories can be efficiently retrieved and updated, ensuring that the most pertinent information remains easily accessible. This approach mirrors the brain's ability to filter and prioritize experiences, focusing on valuable memories while allowing less critical information to fade.

\textbf{2) Context-Based Retrieval} allows memory systems to dynamically recall relevant information based on current needs. Rather than relying solely on explicit keywords, retrieval can be enhanced by leveraging semantic similarity, temporal context, and retrieval frequency. This method improves both the precision and relevance of the information recalled, much like how humans retrieve memories by associating past experiences with present situations.

\textbf{3) Memory consolidation} is also crucial for maintaining LTM for further utilization. Systems must periodically assess the relevance and usage of stored memories, reinforcing essential data through consolidation while gradually deprioritizing less frequently accessed information. This helps avoid issues such as catastrophic forgetting by ensuring critical memories remain intact while the system avoids becoming cluttered with outdated or irrelevant data.

\textbf{4) Self-reflection} enables personalized models to refine their LTM by periodically reviewing stored information. Through this reflective process, general principles can be abstracted from specific experiences, leading to more efficient memory management and retrieval strategies in the future. This self-reflective capacity not only optimizes memory storage but also enhances decision-making and adaptability over time.

Comparing with previous LTM utilization strategies, the proposed multi-agent based LTM management framework are more general to corporate with distinct LLMs. The mentioned four modules/functions can be distributed across different agents with specific tasks. By analyzing user behavior patterns over time, agents can better plan actions and make more informed decisions, resulting in a more adaptive and personalized experience. The integration of these memory-focused processes allows agents to operate cohesively, leveraging their shared knowledge to create a more efficient and human-like system for managing and utilizing long-term memory. 

\subsubsection{Utilizing LTM with RAG to Support Agent Self-evolution}

In previous subsections, we have reviewed the existing research and the multi-agent integration method we proposed to use RAG and ICL for model personalization with LTM. We also want to highlight that LTM can not only facilitate model personalization but also support the model's self-evolution. Take the Agent Hospital study conducted by the Tsinghua University team as an example~\citep{li2024agent}, we will show how the use of LTM helps improve the model’s self-capabilities in a simulacrum medical scenario. The proposed LTM accumulated and utilization method MedAgent-Zero can be mainly divided into three modules: medical records accumulation, medical experience reflection, and RAG-based LTM utilization.

\textbf{1) Medical Records Accumulation.} In this work, the doctor agent first accumulates LTM from successful medical cases to handle future problems. Taking disease diagnosis as an example, after learning the symptoms of a virtual patient, if the doctor agent provides a correct response, this diagnostic process will be saved as a medical record, just like a real-world doctor does, forming text-based LTM data. It is worth noting that even in the real world, the accumulation of medical records is very beneficial for enhancing a doctor's medical capabilities, as it can provide strong decision support when encountering similar issues in the future.

\textbf{2) Medical Experience Reflection.} In the second module, we focus on how the doctor agent accumulates LTM through self-reflection from failed medical cases. Therefore, unlike storing successful medical cases in the memory base directly, we use self-reflection techniques in this module to allow the doctor agent to reflect and summarize after answering the diagnostic problem. The original question, its own response, and the correct response are adopted to generate experience-based LTM data. These data are also text-based, and to ensure their accuracy, we verify if the doctor agent can correctly answer the original question after utilizing the summarized experience (LTM will be dropped once cannot correctly answer). In other words, we designed the construction method for LTM data based on the agent's interaction with different outcomes.

\textbf{3) RAG-based LTM Utilization.} Based on the two types of accumulated LTM data mentioned above, we propose using RAG technology to first retrieve stored cases and experiences when addressing new problems. It is important to note that the retrieval is based on the questions that generated the LTM data. Besides, since no parameter updates are required throughout the process, experience accumulation and application can be conducted online by ICL, making efficient use of the LTM data. As the doctor agent continually acquires valid LTM data during inference, its ability to handle medical questions also improves. Experimental results show that after self-evolving through diagnosing tens of thousands of patients, the doctor agent’s diagnostic capabilities in the respiratory department even surpassed the current SOTA model trained on real-world data.

To summarize, similar to the accumulation and inheritance of human knowledge that can help the development of culture, with appropriate algorithmic support, LTM can also effectively help models in achieving self-capability enhancement, which is a further step in model personalization. Although the handling and application types of LTM in this work still have limitations, it fully demonstrates the potential of this direction. In Section 7, we will provide future optimization directions.


% \subsubsection{Unsolved Challenges}
% At first glance, this new paradigm appears to effectively emulate the function of long-term memory in the human brain. However, despite its theoretical strengths, the limitations of this architecture in practical engineering applications are becoming increasingly evident as research progresses. 

% \begin{itemize}
%     \item \textbf{Encoding:} the current LLM-based architecture does not filter or prioritize information effectively. Human memory encoding is highly selective, focusing on what is relevant or significant for long-term retention. In contrast, LLMs encode data indiscriminately, leading to large amounts of irrelevant or redundant information in the memory system. This not only burdens retrieval processes but also affects the model's ability to use stored information meaningfully.
%     \item \textbf{Storage:}while RAG can theoretically store unlimited data, practical issues arise related to data management. Unlike the human brain, which consolidates memories during rest periods, external databases for LLMs lack mechanisms to automatically organize or consolidate information over time. As a result, data stored in these systems becomes fragmented and increasingly difficult to retrieve efficiently. Furthermore, the reliance on large-scale external storage introduces latency and scalability challenges, which limit the model’s real-time performance.
%     \item \textbf{Retrieval:} LLMs retrieve stored information based on probabilistic token prediction. While this allows dynamic generation, it often retrieves data that is contextually irrelevant or incomplete. Unlike human memory, which is context-driven and associative, LLMs may select data based on superficial similarities. This mismatch leads to inaccurate or inappropriate outputs, especially when dealing with complex or nuanced queries that require deeper semantic connections.
% \end{itemize}

% In essence, the primary limitations of the RAG+ICL architecture stem from its inability to effectively filter, organize, and retrieve information in a way that mimics the efficiency and selectivity of human memory. Without better mechanisms for memory prioritization and consolidation, the system risks becoming overwhelmed by irrelevant data, reducing its ability to provide meaningful and accurate responses.


\subsection{Incorporating LTM by Updating Model Parameters}%Integrate Long-Term Memory with model parameterization}
Another type of strategy for constructing model personalization using LTM is through a parameterized approach, where the accumulated LTM data is transformed into the model's internal parameter memory through model training. The largest difference between this method and the LTM data utilization in RAG and ICL is that it directly modifies the parameters of the foundation model. As a result, it requires a larger data scale, higher implementation costs, and lower update efficiency compared to the former. However, its advantage lies in not needing an explicit LTM management mechanism design, and it can also be completed through single-step inference during the inference.

% A previous survey on memory mechanism in LLM-based agents \citep{zhang2024memoagentsurvey} identifies two primary forms of memory in use: textual form and parametric form. In the textual form, memory is processed explicitly using natural language, while in the parametric form, memory is encoded directly into the model's weights, allowing implicit usage during inference. This distinction can be generalized to our current context: in addition to interacting with LTM data in their respective modalities (e.g., text, sound or video etc) during prompt construction, it is also possible to integrate them directly into LLMs through model training. 
To be more specific, regardless of a foundation model's architecture, the LLM training paradigm can be typically classified into three types: pre-training, instruction tuning, and alignment tuning \citep{zhao2023survey}. This has become a standard approach for many state-of-the-art LLMs \citep{touvron2023llama2, dubey2024llama3, jiang2024mixtral}. Notably, these phases may be iterated multiple times to achieve optimal results. Each of the stages presents a different opportunity for LTM data integration.

\subsubsection{Brief Review of Pre-Training, Instruction Tuning, and Alignment Tuning}

Here, we first briefly review the pre-training, instruction tuning, and alignment tuning of LLMs, which can be used to encode LTM data for model personalization.

\textbf{Pre-training.} Pre-training is generally conducted on large-scale corpora in an unsupervised manner and it is essential for LLMs because it can equip them with extensive world knowledge and a deep understanding of language \citep{brown2020fslearner, zhao2023survey}. 
% One of the two common pre-training tasks \citep{zhao2023survey} is Language Modeling and it is usually used to train decoder-only models such as Llama \citep{touvron2023llama1}, GPT \citep{brown2020fslearner}, and PaLM \citep{Chowdhery2024palm} series. 
The next-token prediction task is commonly used to train decoder-only models, such as Llama \citep{touvron2023llama1} and GPT \citep{brown2020fslearner}, which aims to predict a target token $x_i$ based on the preceding sequence in an auto-regressive manner. In essence, the training objective is to maximize:
\begin{equation}
\mathcal{L} = \sum_{i=1}^n \log P(x_i | x_1,\ldots,x_{i-1}).
\end{equation}
Pre-training typically requires significant computational resources and large-scale data support, while LTM data often faces data sparsity issues. So a candidate method known as continued pre-training can be employed to encode LTM into models. By using a similar loss function, a pre-trained LLM can continue learn new data about specific tasks \citep{parmar2024reuse}, such as recent information \citep{qin2022elle, jang2022conttrainllm} or domain-specific knowledge \citep{colombo2023saulllm, ke2022conttrainllmdomain, Gururangan2020conttraindomain}. Thus, this strategy also works for encoding LTM data. 

Despite continued pre-training enabling LLMs to acquire new knowledge and is particularly useful for integrating LTM data, there is a potential risk of catastrophic forgetting~\citep{parmar2024reuse}. Research shows that the learning rate schedule \citep{gupta2023rewarm, winata2023lradjust} and data distribution \citep{ibrahim2024simplecontpretrainstrat} during the continued pre-training phase can be helpful, as well as updating only a subset of the model's parameters to minimize the impact on the original knowledge~\citep{wu2024llamablockexpansion}.

\textbf{Instruction tuning.} After pre-training, instruction tuning is performed to further enhance their capabilities by fine-tuning the model with instruction instances in a supervised manner. These instances typically consist of a task description ($T$), along with input ($X$) and desired output ($Y$) pairs. LTM data can also be reorganized in this format and be encoded into LLMs. For LLM-orientated training, the instructions (or prompts) ($I$) are usually constructed as $I = T + X$. Therefore the training objective of instruction tuning (in the context of LLM, this is also called Supervised Fine-Tuning (SFT) \citep{ouyang2022rlhf}) that can be formalised as:
\begin{equation}
P\left(Y_1,\ldots, Y_n | I_1,\ldots,I_m\right) = \prod^{n}_{j=1} P \left(Y_j | I_1,\ldots, I_m,Y_1,\ldots,Y_{j-1}\right),
\end{equation}
where $I = \left\{I_1,\ldots,I_m\right\}$ and $Y = \left\{Y_1,\ldots,Y_n\right\}$ are the instruction and output sequence respectively. In essence, the model is trained to predict each token in $Y$ given $I$ and $Y$ so far \citep{shi2024sftloss}. A common loss function for this training objective is simply the negative log-likelihood of the completion tokens:
\begin{equation}
\mathcal{L} = -\log P(Y_1, \ldots, Y_n | I_1,\ldots, I_m) = -\sum_{j=1}^n \log P(Y_j | I_1,\ldots, I_m, Y_1,\ldots, Y_{j-1}).
\end{equation}

For LTM data, this phase presents a prime opportunity for memory integration. Unlike pre-training, only a moderate amount of data (i.e. pairs of ($I$, $Y$)) is required in this phase to significantly influence the model, leading to general performance improvements \citep{zhao2023survey}. As a direct comparison, humans receive a vast amount of real-time events, and they filter these signals to distill valuable information. Only a small portion of this information (i.e. $I$) is stored in human's LTM through repetitive activation and memorization, which can be retrieved and output (i.e. $Y$) later for downstream tasks. To mimic this process, we must curate a refined set of instruction data and train the model iteratively on this smaller set. The quality of this refined information (or data) is crucial in influencing both human and LLM decision-making and performance. Moreover, instruction tuning not only enhances the model’s performance on the trained tasks but also enables LLMs to generalize to unseen tasks \citep{chung2024sftscale}. Additionally, like pre-training, domain-specific knowledge can also be infused into the model, turning it into a subject matter expert. These qualities are highly desirable for effective LTM data utilization, as the final entity should be capable of performing tailored and complex actions following model personalization. Understanding what data accurately reflects LTM is crucial when incorporating them into LLMs. The answer varies depending on the application. For example, in an emotional support chatbot, LTM includes past sessions between users and the chatbot \cite{li2024hello}. In a medical assistant scenario, LTM involves patients' past medical records \citep{zhang2023memory}.

% In several studies exploring the relationship between LTM and LLMs, the concept of memory operations has been frequently discussed \citep{zhang2024memoagentsurvey, wang2024autoagentsurvey, wang2023userbehavsim}. There is a general consensus that two key actions, \textit{memory writing} and \textit{memory reading}, are essential for making memory useful to LLMs or LLM-based agents. Typically, memory writing (or editing) only involves part of the original memory, or leave the original memory intact. Drawing a direct analogy to model parameterization, memory writing and memory reading can be compared to SFT and inference. While fully parameterized fine-tuning (full SFT) is feasible for memory writing, there are alternative approaches that involve training a smaller set of weights \citep{hu2021lora, dettmers2023qlora, gao2023llamaadapterv2} or adding a new segment to the original model layers \citep{liu2023ptunev2, li2021prefixtune}. The former approach acts as a memory adapter attached to the pre-fine-tuned model and can either be fused with the model or used as additional parameters during inference. The latter approach is usually used to increase of the performance on specific tasks. For memory reading, the inference method is closely related to the model's training process and the data used, but the inference module should be aligned with the training phase to ensure that injected memories are retrieved accurately and efficiently.

\textbf{Alignment tuning.} Despite extensive data cleaning, the large volume of pre-training data may still vary in quality, potentially leading to undesired responses \citep{wang2024comprehensive}. Several methods have been proposed to enhance LLMs, particularly in aligning them with human expectations and preferences to enable personalization, which can also be used to encode LTM data after labeling. Reinforcement Learning from Human Feedback (RLHF) \citep{ouyang2022rlhf} and Reinforcement Learning from AI Feedback (RLAIF) \citep{lee2023rlaif} are two prevalent alignment methods. RLHF tunes a reward model that rates different outputs based on human feedback, which is then used to further fine-tune the LLM \citep{christiano2017deep}. In contrast, RLAIF directly links the LLM to a larger, more aligned model for learning. Due to the complexity and overall performance of RLHF, other methods such as Direct Preference Optimization (DPO) \citep{rafailov2024direct}, Knowledge Transfer Optimization (KTO) \citep{kto}, Optimized Reward Preference Optimization (ORPO) \citep{hong2024orpo}, and Simplified Preference Optimization (SimPO) \citep{meng2024simpo} are often employed in different scenarios for alignment tuning. However, although it is technically feasible to adjust model preferences for specific applications or even incorporate domain knowledge in reward models to impart biases \citep{nath2024rmecommerce, lin2024dogerm}, curating a high-quality preference dataset that aligns with the desired LTM remains challenging.

To summarize, model parameterization occurs during all three phases of LLM training, making LTM integration theoretically possible at any stage to achieve model personalization. However, due to constraints such as data availability, training stability, and computational resources, we think that SFT remains the predominant technique for model personalization.

\subsubsection{Model Personalization through Training with LTM Data}
\label{model_personalisation_sft}
Compared to the LTM integration strategies based on RAG and ICL, although the parameterized training encoding method introduced earlier requires more resources, it has significant advantages in terms of input format and inference efficiency. As most current LTM data are in the textual form due to its clearer interpretability, better context control, and ease of implementation \citep{zhang2024memoagentsurvey}, supporting textual LTM requires LLMs to have a sufficiently large context window to incorporate all necessary information during prompt construction. However, decoder-based LLMs are typically constrained by a fixed, limited context window. To address this, significant efforts have been made to extend the context window effectively \citep{chen2023pi, press2022alibi, ding2024longrope, peng2023yarn, zhu2024pose, chen2024longlora, xiong2023longllama} or to process information in parallel \citep{hao2022structprompt, ratner2023parallelwindow}. Despite these advancements, the information stored in LTM can still exceed the capacity of state-of-the-art context windows. Additionally, due to the architecture of transformers \citep{vaswani2017attention}, which serve as the foundation for most LLMs, computational cost increases quadratically with input length. This makes extremely long inputs less practical for some applications. A limited context window necessitates the use of a retriever to select relevant information from a large, manually curated LTM resource, such as a database or vector store \citep{zhong2024memorybank}. This shifts the challenge from the LLM to the design of an effective retriever. Injecting LTM data directly into the model addresses this limitation, as it eliminates the need to include such information in the input prompt. This allows the LLM to focus on the task at hand, with memory retrieval integrated into the model’s inference process. This integration leverages the LLM's advanced language understanding and reasoning capabilities, avoiding dependence on a (usually) less capable external retriever.

If we choose to use training methods to encoder LTM data into LLMs, a vital question is how to decide the data structures and types for training. As we known, in LLM-based agents, short-term memory manages contextual information, while long-term memory stores past experiences, reflections, and profiles. Profiles are arguably one of the most critical components of an agent, directly influencing its functions and interactions \citep{wang2024autoagentsurvey}. Typically, profiles contain basic details such as age, gender, and occupation \citep{park2023stanfordtown}, and may also include traits, interests, and behavioral patterns \citep{wang2023userbehavsim}. While it is possible to fit such descriptions into a prompt, this approach only portrays an average person playing a specific role, lacking the depth needed to reflect an individual’s rich history and experiences \citep{shao2023charllm}. To integrate such data into the model in a unified way, one can use SFT with specially curated datasets. In Character-LLM \citep{shao2023charllm}, training data is constructed not only from profiles but also from experiences and scenarios, enabling LLMs to display more human-like characteristics. Similar works \citep{zhou2023charglm, chen2023haruhi} also fine-tune models using character-specific data derived from past memories and experiences, proving effective in aligning models more closely with their intended personas.

In addition to in-character memory, one of the most crucial aspects of LTM is its associated domain knowledge. It has been well established that LLMs can be significantly enhanced in specific domains through fine-tuning, enabling smaller models to perform on par with, or even surpass, larger models. This is especially evident in domains that require extensive knowledge for complex reasoning and decision-making, such as healthcare, finance, and law \cite{zhao2023survey}. For instance, the Med-PaLM series \citep{singhal2024medpalm1, singhal2024medpalm2}, fine-tuned from the PaLM model \citep{Chowdhery2024palm}, became the first model to pass the U.S. Medical Licensing Examination (USMLE), demonstrating human-expert level proficiency in the medical domain. Similarly, in the field of law, Legal Artificial Intelligence (LegalAI) \citep{zhong2020legalai} has advanced significantly with the advent of LLMs. Fine-tuned models can now perform in-depth legal question-answering, simulating the role of a lawyer \citep{huang2023lawyerllama, cui2023chatlaw}, and efforts are underway to develop intelligent legal service systems \citep{yue2023disclawllm}. In finance, domain-specific fine-tuning has also shown significant promise, as seen in models like BloombergGPT \citep{wu2023bloomberggpt} and FinGPT \citep{yang2023fingpt}. Domain knowledge plays a vital role in model personalization, and these examples demonstrate the feasibility of integrating specialized knowledge, which elevates models beyond their general-purpose capabilities.

% \subsubsection{Memory Operations}

% In several studies exploring the relationship between LTM and LLMs, the concept of memory operations has been frequently discussed \citep{zhang2024memoagentsurvey, wang2024autoagentsurvey, wang2023userbehavsim}. There is a general consensus that two key actions, \textit{memory writing} and \textit{memory} reading, are essential for making memory useful to LLMs or LLM-based agents. Additionally, a third operation, \textit{memory management}, which involves editing or reflecting on memories to generate higher-level insights, is beneficial for the overall design of LTM systems.

% Drawing a direct analogy to model parameterization, memory writing and memory reading can be compared to model training and inference. While fully parameterized training, as discussed earlier, is feasible for memory writing, there are alternative approaches that involve training a smaller set of weights \citep{hu2021lora, dettmers2023qlora, gao2023llamaadapterv2} or adding a new segment to the original model layers \citep{liu2023ptunev2, li2021prefixtune}. The former approach acts as a memory adapter attached to the pre-fine-tuned model and can either be fused with the model or used as additional parameters during inference. The latter approach can further enhance the model's performance in specific tasks. For memory reading, the inference method is closely related to the model's training process and the data used, but the inference module should be aligned with the training phase to ensure that injected memories are retrieved accurately and efficiently.

% Memory editing and management, however, is more challenging in the context of model parameterization. Once deployed, LLMs typically remain static, yet new memories and knowledge are continually emerging. It is, therefore, important to implement mechanisms for continuous learning. In the context of LTM, this involves horizontal continual learning, which refers to continual adaptation across time and domains. This process involves multiple training stages and is prone to the issue of catastrophic forgetting \citep{shi2024continual}. Novel approaches, such as Curlora \citep{fawi2024curlora}, have been proposed to fine-tune LLMs while mitigating forgetting and reducing the number of trainable parameters. This method introduces a unique modification to the CUR decomposition process, using inverted probabilities for column and row selection as implicit regularization and initializing the U matrix as zero, with only the U matrix being fine-tuned.

% \subsubsection{Data Collection and Composition}

% High-quality data plays a more essential part in the training of LLMs compared to the traditional small-scale language models. LLMs' capacities largely rely on the training data and how it has been preprocessed \citep{zhao2023survey}. 

% After defining the long term memory data which can be used for model training, the training data needs to go through a serios of preprocessing steps including removing noise, handingling outliers, addressing imbalances, text preprocessing and dealing with ambiguities \citep{minaee2024large}. 

% With the collected and filtered raw data, prompt engineering is often employed to further re-write some of the data to better train the model. For example, by incorporating Chain of Thought (CoT)\citep{wei2022chain} data, the model learns to generate multi-step reasoning capabilities, automatically retrieving more relevant context from the long term memory.

% \textbf{Full-Scale Fine-Tuning} involves fully fine-tuning the model with all available data to incorporate long-term memory into the personalized model.

% % PEFT
% \textbf{Parameter-Efficient Fine-Tuning (PEFT)} methods enable efficient adaptation of large pretrained models by fine-tuning only a small number of extra parameters instead of the full parameters of the models. 

% \citep{zhang2023memory} introduced a novel memory mechanism inspired by neuroscience, and along with a PEFT training strategy to achieve LLM-based medical assistant personalization.

% \citep{wang2024augmenting} proposed a LongMem framework which slices long-text inputs and storing them in a Memory bank. It also designs a side network that integrates memory through QKV (Query, Key, Value) fusion to address the problem of memory staleness.

% \subsubsection{Personalization}

% Personalization can be implemented in both training and inference stage. The long term memory data used for training the model enables the retrieval of users' memory.With the models fine-tuned on personlized long term memory, users are able to enjoy long-term companionship and personalized interactions with chatbots\citep{li2024hello}. For inference stage, prompt engineering is often employed for more customized and personized response. More details can be seen in Chapter X.

\subsection{Incorporatin LTM Data with Mixed Strategy}
Since using LTM data solely as an external knowledge base or as additional training data each has its own advantages and limitations, a simple idea is whether we can integrate these two methods (RAG with ICL and SFT) to leverage their strengths and achieve more effective model personalization. 
Recent works on RAG also see an increase in fine-tuning models at each stage of RAG: retrieval, augmentation, and generation. By focusing on fine-tuning, we can significantly enhance an RAG system’s efficiency and effectiveness in handling LTM data. 

\subsubsection{Fine-Tuning in the Retrieval Stage}
The retrieval stage in RAG systems involves selecting relevant documents or knowledge chunks from external sources to boost the model's intrinsic knowledge. Fine-tuning the retriever model at this stage optimizes its ability to retrieve more relevant, domain-specific information. 

By fine-tuning the retriever with LTM data, the precision of retrieving highly relevant content improves. In fields such as law or medicine, this ensures that the retriever pulls accurate and specialized content, increasing relevance and reducing noise during the retrieval process. This addresses the limitations of generic models, which may retrieve unrelated or less useful data \citep{gao2023ragllmsurvey}. This process is often applied to embedding models to align the representations of both the query and external documents with the domain's vocabulary and semantics. This alignment enhances retrieval effectiveness by improving semantic similarity matching. Moreover, fine-tuning has been used to align the retriever with the generator. One such method is the LM-Supervised Retriever (LSR), where the output of LLMs is used to train the retriever in a feedback loop \citep{gao2023ragllmsurvey}. For instance, REPLUG LSR \citep{shi2023replug} trains the retriever to select documents that can reduce the perplexity of the LLM's output sequences.

\subsubsection{Fine-Tuning in the Augmentation Stage}

The augmentation stage in RAG systems integrates retrieved LTM data with the model's existing knowledge to create a comprehensive context for generating an informed response. Fine-tuning can optimize the integration and selection of relevant information at this stage. Since the augmentation stage acts as an intermediary between retrieval and generation, fine-tuning can be applied to the retriever, the generator, or as an additional module in between.

For instance, fine-tuning enhances contextual filtering and selection by eliminating redundant or irrelevant information from the retrieved documents. This ensures that only the most pertinent data is used in the generation stage and this improves the quality of responses. A notable example is Self-RAG \citep{asai2023selfrag}, which uses reflection tokens to indicate whether retrieved documents are relevant to the query, whether the generated responses are supported by the documents, or whether the response effectively addresses the query. This approach significantly improves and streamlines the augmentation process. Additionally, models can optimize their augmentation strategies through document grounding, particularly when handling large volumes of documents. Fine-tuned models are better equipped to identify relevant and critical information from the retrieved content, resulting in more accurate response generation and reducing the likelihood of hallucination \citep{huang2020llmcite}.

\subsubsection{Fine-Tuning in the Generation Stage}

The generation stage is where LLM, enhanced by the retrieved context, produces the final response. Fine-tuning at this stage improves the quality of the generated text and ensures alignment with the desired style, tone, and factual accuracy. For instance, fine-tuning enables the LLM to conform to specific data formats and enforce a particular response style, as instructed. This technique is especially useful for equipping LLMs with function-calling capabilities and tool usage \citep{patil2023gorilla}.

Fine-tuning also allows the model to be customized for specific tasks or domains, ensuring that the generated content adheres to domain-specific norms and conventions. For example, in medical applications, fine-tuning helps the model generate clinically appropriate responses, while in legal tasks, it ensures adherence to legal terminology and reasoning. Additionally, the Chain-of-Thought process \citep{wei2022chain} can be integrated into model generation, guiding the model through complex reasoning and facilitating connections between relevant knowledge in the retrieved documents \citep{li2024rtghop}.


To summarize, the integrated LTM utilization method can better combine the respective advantages of both strategies, thereby ensuring efficient data usage while achieving accurate personalized generation. However, such a strategy still faces a series of challenges in practice, such as how to determine the frequency of SFT to balance efficiency and effectiveness.

==> old_sections/00_abstract.tex <==
\begin{abstract}
We introduce Transfusion, a recipe for training a multi-modal model over discrete and continuous data.
Transfusion combines the language modeling loss function (next token prediction) with diffusion to train a single transformer over mixed-modality sequences.
We pretrain multiple Transfusion models up to 7B parameters from scratch on a mixture of text and image data, establishing scaling laws with respect to a variety of uni- and cross-modal benchmarks.
Our experiments show that Transfusion scales significantly better than quantizing images and training a language model over discrete image tokens.
By introducing modality-specific encoding and decoding layers, we can further improve the performance of Transfusion models, and even compress each image to just 16 patches.
We further demonstrate that scaling our Transfusion recipe to 7B parameters and 2T multi-modal tokens produces a model that can generate images and text on a par with similar scale diffusion models and language models, reaping the benefits of both worlds.
\end{abstract}

==> old_sections/01_intro.tex <==
\section{Introduction}

Multi-modal generative models need to be able to perceive, process, and produce both discrete elements (such as text or code) and continuous elements (e.g. image, audio, and video data).
While language models trained on the next token prediction objective dominate discrete modalities \citep{gpt4, llama3}, diffusion models \citep{ho2020denoising, ldm} and their generalizations \citep{lipman2022flow} are the state of the art for generating continuous modalities \citep{dai2023emu, sd3, bar2024lumiere}.
Many efforts have been made to combine these approaches, including extending a language model to use a diffusion model as a tool, either explicitly \citep{liu2023llavaplus} or by grafting a pretrained diffusion model onto the language model \citep{dong2023dreamllm,koh2024generating}.
Alternatively, one can quantize the continuous modalities \citep{vqvae} and train a standard language model over discrete tokens \citep{dalle, yu2022scaling, yu2023scaling}, simplifying the model's architecture at the cost of losing information.
In this work, we show it is possible to fully integrate both modalities, with no information loss, by training a single model to both predict discrete text tokens and diffuse continuous images.

We introduce \textbf{Transfusion}, a recipe for training a model that can seamlessly generate discrete and continuous modalities.
We demonstrate Transfusion by pretraining a transformer model on 50\% text and 50\% image data using a different objective for each modality: next token prediction for text and diffusion for images.
The model is exposed to both modalities and loss functions at each training step.
Standard embedding layers convert text tokens to vectors, while patchification layers represent each image as a sequence of patch vectors.
We apply causal attention for text tokens and bidirectional attention for image patches.
For inference, we introduce a decoding algorithm that combines the standard practices of text generation from language models and image generation from diffusion models.
Figure~\ref{fig:transfusion} illustrates Transfusion.

In a controlled comparison with Chameleon's discretization approach \citep{team2024chameleon}, we show that Transfusion models scale better in every combination of modalities.
In text-to-image generation, we find that Transfusion exceeds the Chameleon approach at less than a third of the compute, as measured by both FID and CLIP scores.
When controlling for FLOPs, Transfusion achieves approximately 2$\times$ lower FID scores than Chameleon models.
We observe a similar trend in image-to-text generation, where Transfusion matches Chameleon at 21.8\% of the FLOPs.
Surprisingly, Transfusion is also more efficient at learning text-to-text prediction, achieving perplexity parity on text tasks around 50\% to 60\% of Chameleon's FLOPs.

Ablation experiments reveal critical components and potential improvements for Transfusion.
We observe that the intra-image bidirectional attention is important, and that replacing it with causal attention hurts text-to-image generation.
We also find that adding U-Net down and up blocks to encode and decode images enables Transfusion to compress larger image patches with relatively small loss to performance, potentially decreasing the serving costs by up to 64$\times$.

Finally, we demonstrate that Transfusion can generate images at similar quality to other diffusion models.
We train from scratch a 7B transformer enhanced with U-Net down/up layers (0.27B parameters) over 2T tokens: 1T text tokens, and approximately 5 epochs of 692M images and their captions, amounting to another 1T patches/tokens.
Figure~\ref{fig:samples1} shows some generated images sampled from the model.
On the GenEval \citep{ghosh2023geneval} benchmark, our model outperforms other popular models such as DALL-E 2 and SDXL; unlike those image generation models, it can generate text, reaching the same level of performance as Llama 1 on text benchmarks.
Our experiments thus show that Transfusion is a promising approach for training truly multi-modal models.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{pics/model_diagram-crop.pdf}
\caption{A high-level illustration of Transfusion. A single transformer perceives, processes, and produces data of every modality. Discrete (text) tokens are processed autoregressively and trained on the \textcolor[HTML]{2171c7}{next token prediction} objective. Continuous (image) vectors are processed together in parallel and trained on the \textcolor[HTML]{e69500}{diffusion} objective. Marker BOI and EOI tokens separate the modalities.}
\label{fig:transfusion}
\end{figure}






==> old_sections/02_background.tex <==
\section{Background}
\label{sec:background}

Transfusion is a single model trained with two objectives: language modeling and diffusion.
Each of these objectives represents the state of the art in discrete and continuous data modeling, respectively. 
This section briefly defines these objectives, as well as background on latent image representations.


\subsection{Language Modeling}
\label{sec:lm}

Given a sequence of discrete tokens $y = y_1, ..., y_n$ from a closed vocabulary $V$, a language model predicts the probability of the sequence $P(y)$.
Standard language models decompose $P(y)$ into a product of conditional probabilities $\prod_{i=1}^n P_\theta(y_i|y_{<i})$.
This creates an autoregressive classification task, where the probability distribution of each token $y_i$ is predicted conditioned on the prefix of a sequence $y_{<i}$ using a single distribution $P_\theta$ parameterized by $\theta$.
The model can be optimized by minimizing the cross-entropy between $P_\theta$ and the empirical distribution of the data, yielding the standard next-token prediction objective, colloquially referred to as \textit{LM loss}:
\begin{equation}
\mathcal{L}_{\text{LM}} = \mathbb{E}_{y_i} \big[ - \log P_\theta (y_i | y_{<i}) \big]
\end{equation}
Once trained, language models can also be used to generate text by sampling token by token from the model distribution $P_\theta$, typically using temperature and top-p truncation.


\subsection{Diffusion}
\label{sec:diffusion}

Denoising diffusion probabilistic models (a.k.a. \textit{DDPM} or \textit{diffusion models}) operate on the principle of learning to reverse a gradual noise-addition process \citep{ho2020denoising}.
Unlike language models that typically work with discrete tokens ($y$), diffusion models operate over continuous vectors ($\mathbf{x}$), making them particularly suited for tasks involving continuous data like images.
The diffusion framework involves two processes: a forward process that describes how the original data is turned into noise, and a reverse process of denoising that the model learns to perform.

\paragraph{Forward Process}
From a mathematical perspective, the forward process defines how the noised data (which serves as the model input) is created.
Given a data point $\mathbf{x}_0$, \citet{ho2020denoising} define a Markov chain that gradually adds Gaussian noise over $T$ steps, creating a sequence of increasingly noisy versions $\mathbf{x}_1, \mathbf{x}_2, ..., \mathbf{x}_T$.
Each step of this process is defined by $q(\mathbf{x}_t | \mathbf{x}_{t-1}) = \mathcal{N}(\mathbf{x}_t; \sqrt{1 - \beta_t}\mathbf{x}_{t-1}, \beta_t\mathbf{I})$, where $\beta_t$ increases over time according to a predefined noise schedule (see below).
This process can be reparameterized in a way that allows us to directly sample $\mathbf{x}_t$ from $\mathbf{x}_0$ using a single sample of Gaussian noise $\boldsymbol{\epsilon} \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$:
\begin{equation}
\mathbf{x}_t = \sqrt{\bar{\alpha}_t}\mathbf{x}_0 + \sqrt{1-\bar{\alpha}_t}\boldsymbol{\epsilon}
\label{eq:forward}
\end{equation}
Here, $\bar{\alpha}_t = \prod_{s=1}^t (1-\beta_s)$, providing a useful abstraction over the original Markov chain.
In fact, both the training objective and the noise scheduler are eventually expressed (and implemented) in these terms.

\paragraph{Reverse Process}
The diffusion model is trained to perform the reverse process $p_\theta(\mathbf{x}_{t-1}|\mathbf{x}_t)$, learning to denoise the data step by step.
There are several ways to do so; in this work, we follow the approach of \citet{ho2020denoising} and model the Gaussian noise $\boldsymbol{\epsilon}$ in Equation~\ref{eq:forward} as a proxy for the cumulative noise at step $t$.
Specifically, a model $\epsilon_\theta(\cdot)$ with parameters $\theta$ is trained to estimate the noise $\boldsymbol{\epsilon}$ given the noised data $\mathbf{x}_t$ and timestep $t$.
In practice, the model often conditions on additional contextual information $c$, such as a caption when generating an image.
The parameters of the noise prediction model are thus optimized by minimizing the mean squared error loss:
\begin{equation}
\mathcal{L}_{\text{DDPM}} = \mathbb{E}_{\mathbf{x}_0, t, \boldsymbol{\epsilon}}\big[||\boldsymbol{\epsilon} - \boldsymbol{\epsilon}_{\theta}(\mathbf{x}_t, t, c)||^2\big]
\end{equation}

\paragraph{Noise Schedule}
When creating a noised example $\mathbf{x}_t$ (Equation~\ref{eq:forward}), $\bar{\alpha}_t$ determines the variance of the noise for timestep $t$.
In this work, we adopt the commonly used cosine scheduler~\cite{nichol2021improved}, which largely follows $\sqrt{\bar{\alpha}_t} \approx \cos(\frac{t}{T}\cdot\frac{\pi}{2})$ with some adjustments.

\paragraph{Inference}
Decoding is done iteratively, pealing away some of the noise at each step.
Starting with pure Gaussian noise at $\mathbf{x}_T$, the model $\boldsymbol{\epsilon}_{\theta}(\mathbf{x}_t, t, c)$ predicts the noise accumulated at timestep $t$.
The predicted noise is then scaled according to the noise schedule, and the proportional amount of predicted noise is removed from $\mathbf{x}_t$ to produce $\mathbf{x}_{t-1}$.
In practice, inference is done over fewer timesteps than training.
Classifier-free guidance (CFG)~\citep{ho2022classifier} is often used to improve generation by contrasting the prediction of the model conditioned on the context $c$ with the unconditioned prediction, at the cost of doubling the computation.


\subsection{Latent Image Representation}
\label{sec:vae}

Early diffusion models worked directly in pixel space \citep{ho2020denoising}, but this proved computationally expensive.
Variational autoencoders (VAEs) \citep{kingma2013auto} can save compute by encoding images into a lower-dimensional latent space. 
Implemented as deep CNNs, modern VAEs are trained on a combination of reconstruction and regularization losses \citep{esser2021taming}, allowing downstream models like latent diffusion models (LDMs) \citep{ldm} to operate efficiently on compact image patch embeddings; e.g. represent every 8$\times$8 pixel patch as an 8-dimensional vector.
For autoregressive language modeling approaches \citep{dalle, yu2022scaling}, images must be discretized.
Discrete autoencoders, such as vector-quantized VAEs (VQ-VAE) \citep{vqvae}, achieve this by introducing a quantization layer (and related regularization losses) that maps continuous latent embeddings to discrete tokens.


==> old_sections/03_method.tex <==
\section{Transfusion}
\label{sec:method}

\begin{figure}[t]
  \centering
  \begin{minipage}[b]{0.47\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/model_vision-crop.pdf}
    \caption{We convert images to and from latent representations using a pretrained VAE, and then into patch representations with either a simple linear layer or U-Net down blocks.}
    \label{fig:encdec}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.47\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/attention_mask-crop.pdf}
    \caption{Expanding on the causal mask, Transfusion allows patches of the same image to condition on each other.}
    \label{fig:attention}
  \end{minipage}
\end{figure}

% \todo{1) Remove in/out tokens from the image. 2) Encoder/Decoder capitalized. 3) Noising capitalized. 4) U-Net Down / U-Net Up   (capitalization, no "blocks").}
Transfusion is a method for training a single unified model to understand and generate both discrete and continuous modalities.
Our main innovation is demonstrating that we can use separate losses for different modalities -- language modeling for text, diffusion for images -- over shared data and parameters.
Figure~\ref{fig:transfusion} illustrates Transfusion.

\paragraph{Data Representation}
We experiment with data spanning two modalities: discrete text and continuous images.
Each text string is tokenized into a sequence of discrete tokens from a fixed vocabulary, where each token is represented as an integer.
Each image is encoded as latent patches using a VAE (see \S\ref{sec:vae}), where each patch is represented as a continuous vector; the patches are sequenced left-to-right top-to-bottom to create a sequence of patch vectors from each image.\footnote{While our canonical setting uses a VAE following latent diffusion models, we were also able to demonstrate Transfusion using raw pixel representations in preliminary experiments.}
For mixed-modal examples, we surround each image sequence with special \textit{beginning of image} (BOI) and \textit{end of image} (EOI) tokens before inserting it to the text sequence;
thus, we arrive at a single sequence potentially containing both discrete elements (integers representing text tokens) and continuous elements (vectors representing image patches).

\paragraph{Model Architecture}
The vast majority of the model's parameters belong to a single transformer, which processes every sequence, regardless of modality.\footnote{We follow Llama's \citep{touvron2023llama} flavor of the transformer block, which includes the SwiGLU activation function~\citep{shazeer2020glu} and RoPE~\citep{su2024roformer}.}\footnote{While we use the transformer architecture in this work, Transfusion could potentially work with other architectures too, despite its name.}
The transformer takes a sequence of high-dimensional vectors in $\mathbb{R}^d$ as input, and produces similar vectors as output.
To convert our data into this space, we use lightweight modality-specific components with unshared parameters.
For text, these are the embedding matrices, converting each input integer to vector space and each output vector into a discrete distribution over the vocabulary.
For images, we experiment with two alternatives for compressing local windows of $k \times k$ patch vectors into a single transformer vector (and vice versa): (1) a simple linear layer,\footnote{We add an embedding of the timestep $t$ to every patch vector before the linear layer.} and (2) up and down blocks of a U-Net \citep{nichol2021improved,saharia2022photorealistic}.\footnote{We replace the U-Net's AdaLayerNorm with regular layer norm in our implementation.}
Figure~\ref{fig:encdec} illustrates the overall architecture.

\paragraph{Transfusion Attention}
Language models typically use causal masking to efficiently compute the loss and gradients over an entire sequence in a single forward-backward pass without leaking information from future tokens.
While text is naturally sequential, images are not, and are usually modeled with unrestricted (bidirectional) attention.
Transfusion combines both attention patterns by applying causal attention to every element in the sequence, and bidirectional attention within the elements of each individual image.
This allows every image patch to attend to every other patch within the same image, but only attend to text or patches of other images that appeared previously in the sequence.
We find that enabling intra-image attention significantly boosts model performance (see \S\ref{sec:ablations}).
Figure~\ref{fig:attention} shows an example Transfusion attention mask.

\paragraph{Training Objective}
To train our model, we apply the language modeling objective $\mathcal{L}_\text{LM}$ to predictions of text tokens and the diffusion objective $\mathcal{L}_\text{DDPM}$ to predictions of image patches.
LM loss is computed per token,\footnote{When the input is a BOI token, we do not compute any loss.} while diffusion loss is computed per image, which may span multiple elements (image patches) in the sequence.
Specifically, we add noise $\boldsymbol{\epsilon}$ to each input latent image $\mathbf{x}_0$ according to the diffusion process to produce $\mathbf{x}_t$ before patchification, and then compute the image-level diffusion loss.\footnote{Ergo, downstream tokens condition on noisy images during training. See \S\ref{sec:noise} for further discussion.}
We combine the two losses by simply adding the losses computed over each modality with a balancing coefficient $\lambda$:
\begin{equation}
\mathcal{L}_\text{Transfusion} = \mathcal{L}_\text{LM} + \lambda \cdot \mathcal{L}_\text{DDPM}
\label{eq:transfusion}
\end{equation}

This formulation is a specific instantiation of a broader idea: combining a discrete distribution loss with a continuous distribution loss to optimize the same model.
We leave further exploration of this space, such as replacing diffusion with flow matching \citep{lipman2022flow}), to future work.

\paragraph{Inference}
Reflecting the training objective, our decoding algorithm also switches between two modes: LM and diffusion.
In \textit{LM mode}, we follow the standard practice of sampling token by token from the predicted distribution.
When we sample a BOI token, the decoding algorithm switches to \textit{diffusion mode}, where we follow the standard procedure of decoding from diffusion models.
Specifically, we append a pure noise $\mathbf{x}_T$ in the form of $n$ image patches to the input sequence (depending on the desired image size), and denoise over $T$ steps.
At each step $t$, we take the noise prediction and use it to produce $\mathbf{x}_{t-1}$, which then overwrites $\mathbf{x}_{t}$ in the sequence; i.e. the model always conditions on the last timestep of the noised image and cannot attend to previous timesteps.
Once the diffusion process has ended, we append an EOI token to the predicted image, and switch back to LM mode.
This algorithm enables the generation of any mixture of text and image modalities.


==> old_sections/04_experiments.tex <==
\section{Experiments}

We demonstrate in a series of controlled experiments that Transfusion is a viable, scalable method for training a unified multi-modal model.


\subsection{Setup}
\label{sec:setup}

\paragraph{Evaluation}
We evaluate model performance on a collection of standard uni-modal and cross-modal benchmarks (Table~\ref{tab:benchmarks}).
For text-to-text, we measure perplexity on 20M held-out tokens from Wikipedia and the C4 corpus \citep{t5}, as well as accuracy on the pretraining evaluation suite of Llama 2 \citep{llama2}.\footnote{The Llama 2 evaluation suite includes HellaSwag~\citep{zellers2019hellaswag}, PIQA~\citep{bisk2020piqa}, SIQA~\citep{sap2019socialiqa}, WinoGrande~\citep{sakaguchi2021winogrande}, ARC-e and -c~\citep{clark2018think}, and BoolQ~\citep{clark2019boolq}. We report the average 0-shot task accuracy on these benchmarks.}
For text-to-image, we use the MS-COCO benchmark \citep{Eval_mscoco}, where we generate images on randomly selected 30k prompts from validation set and measure their photo-realism using zero-shot Frechet Inception Distance (FID) \citep{fid} as well as their alignment with the prompts using CLIP score \citep{clip}.\footnote{We follow common practice for ablations and use only 5k examples to compute FID and CLIP in \S\ref{sec:ablations}.}
We also evaluate the model's ability to generate image captions; we report CIDEr \citep{cider} scores on the Karpathy test split of MS-COCO \citep{Eval_mscoco}.
These evaluations provide signal for investigation scaling laws (\S\ref{sec:simple}) and ablations (\S\ref{sec:ablations}).
To compare with recent literature in diffusion models, we evaluate our largest scale model (\S\ref{sec:enhanced}) also on GenEval \citep{ghosh2023geneval}, a benchmark that examines a model's ability to generate an accurate depiction of the prompt.

\begin{table}[t]
\centering
\begin{minipage}[b]{0.56\textwidth}
\small
\centering
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Input} & \textbf{Output} & \textbf{Benchmark} & \textbf{Metric} \\
\midrule
\multirow{3}{*}{Text} & \multirow{3}{*}{Text} & Wikipedia & Perplexity ($\downarrow$) \\
& & C4 & Perplexity ($\downarrow$) \\
& & Llama 2 Eval Suite & Accuracy ($\uparrow$) \\
\midrule
Image & Text & MS-COCO 5k & CIDEr ($\uparrow$) \\
\midrule
\multirow{2}{*}{Text} & \multirow{2}{*}{Image} & MS-COCO 30k & FID ($\downarrow$), CLIP ($\uparrow$) \\
& & GenEval & GenEval score ($\uparrow$) \\
\bottomrule \\
\end{tabular}
\caption{An overview of the evaluation suite used in this work.}
\label{tab:benchmarks}
\end{minipage}
\hfill
\begin{minipage}[b]{0.41\textwidth}
\small
\centering
\begin{tabular}{@{}lrrr@{}}
\toprule
\textbf{Size} & \textbf{Layers} & \textbf{Emb Dim} & \textbf{Att Heads} \\
\midrule
0.16B & 16 & 768  & 12 \\
0.37B & 24 & 1024 & 16 \\
0.76B & 24 & 1536 & 24 \\
1.4B  & 24 & 2048 & 16 \\
7B    & 32 & 4096 & 32 \\
\bottomrule \\
\end{tabular}
\caption{Model sizes and configurations for both Transfusion and baselines.}
\label{tab:models}
\end{minipage}
\end{table}

\paragraph{Baseline}
At the time of writing, the prominent open-science method for training a single mixed-modal model that can generate both text and images is to quantize images into discrete tokens, and then model the entire token sequence with a standard language model \citep{dalle, yu2022scaling, yu2023scaling}.
We follow the recipe of Chameleon \citep{team2024chameleon} to train a family of data- and compute-controlled baseline models, which we can directly compare to our Transfusion models.
The key difference between Chameleon and Transfusion is that while Chameleon discretizes images and processes them as tokens, Transfusion keeps images in continuous space, removing the quantization information bottleneck.
To further minimize any confounding variables, we train the VAEs for Chameleon and Transfusion using exactly the same data, compute, and architecture, with the only differentiator being the quantization layer and codebook loss of Chameleon's VQ-VAE (see details below).
Chameleon also deviates from the Llama transformer architecture, adding query-key normalization, post-normalization, denominator loss, and a lower learning rate of 1e-4 to manage training instability, which incur an efficiency cost (see \S\ref{sec:simple}).\footnote{Removing these deviations in preliminary experiments encountered optimization instabilities in Chameleon.}

\paragraph{Data}
For almost all of our experiments, we sample 0.5T tokens (patches) from two datasets at a 1:1 token ratio.
For text, we use the Llama 2 tokenizer and corpus \citep{llama2}, containing 2T tokens across a diverse distribution of domains.
For images, we use a collection of 380M licensed Shutterstock images and captions.
Each image is center-cropped and resized to produce a 256$\times$256 pixel image.\footnote{Depending on the compression rate of the patch encoder (see Model Architecture in \S\ref{sec:method}), each image will be represented by either 1024, 256, 64, or 16 elements in the sequence. Since the text/image ratio is constant during training, higher compression rates enable training on more images in total, at the cost of less compute per image.}
We randomly order the image and captions, ordering the caption first 80\% of the time.

In one experiment (\ref{sec:enhanced}) we scale up the total training data to 2T tokens (1T text tokens and about 3.5B caption-image pairs at 256 patches per image).
To diversify, we add 220M publicly available images with captions, prefiltered to not contain people.
To rebalance the distribution, we upsample 80M Shutterstock images containing people.
We also add data from Conceptual 12M (CC12M) \citep{cc12m}, reaching a total mixture of 692M image-caption pairs per epoch.
Finally, we upweight the portion of high-aesthetic images in the last 1\% of the training schedule.

\paragraph{Latent Image Representation}
We train a 86M parameter VAE following \citet{esser2021taming}.
We use a CNN encoder and decoder, and latent dimension 8.
The training objective is combines reconstruction and regularization losses.\footnote{See Appendix~\ref{sec:vae_details} for details.}
Our implementation reduces an image of 256$\times$256 pixels to a 32$\times$32$\times $8 tensor, where each latent 8-dimensional latent pixel represents (conceptually) an 8$\times$8 pixel patch in the original image, and trains for 1M steps.
For VQ-VAE training, we follow the same setup described for VAE training, except we replace $\mathcal{L}_{\text{KL}}$ with the standard codebook commitment loss with $\beta = 0.25$ \citep{vqvae}. We use a codebook of 16,384 token types.

\paragraph{Model Configuration}
To investigate scaling trends, we train models at five different sizes -- 0.16B, 0.37B, 0.76B, 1.4B, and 7B parameters -- following the standard settings from Llama \citep{touvron2023llama}.
Table~\ref{tab:models} describes each setting in detail.
In configurations that use linear patch encoding (\S\ref{sec:simple} and \S\ref{sec:ablations}), the number of additional parameters is insignificant, accounting for fewer than 0.5\% of total parameters in every configuration.
When using U-Net patch encoding (\S\ref{sec:ablations} and \S\ref{sec:enhanced}), these parameters add up to 0.27B additional parameters across all configurations; while this is a substantial addition of parameters to smaller models, these layers amount to only a 3.8\% increase of the 7B configuration, almost identical to the number of parameters in the embedding layers.

\paragraph{Optimization}
We randomly initialize all model parameters, and optimize them using AdamW ($\beta_1=$0.9, $\beta_2=$0.95, $\epsilon=$1e-8) with a learning rate of 3e-4, warmed up for 4000 steps and decaying to 1.5e-5 using a cosine scheduler.
We train on sequences of 4096 tokens in batches of 2M tokens for 250k steps, reaching 0.5T tokens in total.
In our large-scale experiment (\S\ref{sec:enhanced}), we train with a batch size of 4M tokens over 500k steps, totalling 2T tokens.
We regularize with weight decay of 0.1 and clip gradients by norm (1.0).
We set the $\lambda$ coefficient in the Transfusion objective (Equation~\ref{eq:transfusion}) to 5 following preliminary experiments;
we leave further tuning of $\lambda$ to future work.

\paragraph{Inference}
In text mode, we use greedy decoding for generating text.
Ranked classification is used for the Llama evaluation suite.
For image generation, we follow the standard of 250 diffusion steps (the model is trained on 1,000 timesteps).
We follow Chameleon and use CFG with a coefficient of 5 in the controlled comparison experiments (\S\ref{sec:simple}).
This value is suboptimal for Transfusion, and so we use a CFG coefficient of 3 throughout the ablation experiments (\S\ref{sec:ablations}), and follow the standard practice of tuning the coefficient for each benchmark in our large scale experiment (\S\ref{sec:enhanced}).


\subsection{Controlled Comparison with Chameleon}
\label{sec:simple}

We run a series of controlled experiments to compare Transfusion with Chameleon at different model sizes ($N$) and token counts ($D$), using the combination of both as a proxy for FLOPs ($6ND$).\footnote{Since Transfusion uses continuous representations of images, it can express a single image with significantly fewer tokens, shortening the average document length and thus the overall quadratic price of attention. Since this fact favors Transfusion, we remove this confounder by using the theoretical FLOP calculation.}
For simplicity and parameter control, the Transfusion variant in these experiments uses simple linear image encoder/decoder with patch size 2$\times$2, as well as bidirectional attention.
For each benchmark, we plot all results on a log-metric over log-FLOPs curve and regress linear trendlines.\footnote{The smaller Chameleon models perform poorly on image generation and understanding tasks, leading to outlier results that do not correlate with the emerging scaling law of larger Chameleon models. We therefore define minimal performance thresholds below which we remove datapoints: $\leq$100 FID, $\geq$17 CLIP, $\geq$4 CIDEr.}
We also estimate relative compute efficiency by measuring the parity FLOP ratio: the ratio between the number of FLOPs required by Transfusion and Chameleon to reach the same level of performance.

Figure~\ref{fig:controlled} visualizes the scaling trends,
and Table~\ref{tab:controlled} shows the results of the largest models in this controlled setting and their estimated parity FLOP ratio.
In every benchmark, Transfusion consistently exhibits better scaling laws than Chameleon.
While the lines are close to parallel, there is a significant gap in Transfusion's favor.
The difference in compute efficiency is particularly striking in image generation, where FID Transfusion achieves parity with Chameleon using 34$\times$ less compute.

Surprisingly, text-only benchmarks also reveal better performance with Transfusion, even though both Transfusion and Chameleon model text in the same way.
We investigate this phenomenon by ablating the various changes leading up to Transfusion and Chameleon from the original Llama 2 recipe.
Table~\ref{tab:text_analysis} shows that while Transfusion does come at a non-zero cost to text performance, the Chameleon recipe suffers from both the stability modifications made to the architecture and from the introduction of image tokens.
Training on quantized image tokens degrades text performance more than diffusion on all three benchmarks.
One hypothesis is that this stems from the competition between text and image tokens in the output distribution;
alternatively, it is possible that diffusion is more efficient at image generation and requires fewer parameters, allowing Transfusion models to use more capacity than Chameleon to model text.
We leave further investigation of this phenomenon to future research.

\begin{figure}[!t]
  \centering
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/C4.pdf}
    \caption{C4 Perplexity}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/wikipedia.pdf}
    \caption{Wikipedia Perplexity}
  \end{subfigure}

  \vspace{1em}

  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/task.pdf}
    \caption{Llama 2 Eval Suite Accuracy}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/CIDER.pdf}
    \caption{MS-COCO 5k CIDEr}
  \end{subfigure}
  
  \vspace{1em}

  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/FID.pdf}
    \caption{MS-COCO 30k FID}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/CLIP.pdf}
    \caption{MS-COCO 30k CLIP}
  \end{subfigure}
  \caption{Performance of Transfusion and Chameleon models at different scales, controlled for parameters, data, and compute. All axes are logarithmic.}
  \label{fig:controlled}
\end{figure}

\vfill

\begin{table}[!b]
\small
\centering
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{C4}} & \multicolumn{1}{c}{\textbf{Wiki}} & \multicolumn{1}{c}{\textbf{Llama}} & \multicolumn{3}{c}{\textbf{MS-COCO}} \\
& \textbf{PPL} ($\downarrow$) & \textbf{PPL} ($\downarrow$) & \textbf{Acc} ($\uparrow$) & \textbf{CDr} ($\uparrow$) & \textbf{FID} ($\downarrow$) & \textbf{CLIP} ($\uparrow$) \\
\midrule
Transfusion & \textbf{7.72} & \textbf{4.28} & \textbf{61.5}  & \textbf{27.2}  & \textbf{16.8} & \textbf{25.5} \\
Chameleon   & 8.41 & 4.69 & 59.1  & 18.0    & 29.6   & 24.3 \\
\midrule
Parity FLOP Ratio & 0.489 & 0.526 & 0.600 & 0.218 & 0.029 & 0.319 \\
\bottomrule \\
\end{tabular}
\caption{Performance of the largest (7B) Transfusion and Chameleon models in a controlled setting. Both models were trained on 0.5T tokens. \textbf{Parity FLOP Ratio} is the relative amount of Transfusion FLOPs needed to match the results of Chameleon 7B.}
\label{tab:controlled}
\end{table}

\begin{table}[t]
\small
\centering
\begin{tabular}{@{}lllrrr@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} & & \multirow{2}{*}{\textbf{Batch}} & \multicolumn{1}{c}{\textbf{C4}} & \multicolumn{1}{c}{\textbf{Wiki}} & \textbf{Llama} \\
& & & \textbf{PPL} ($\downarrow$)   & \textbf{PPL} ($\downarrow$)  & \textbf{Acc} ($\uparrow$) \\
\midrule
Llama 2      &                                                   & 1M Text Tokens            & 10.1 & 5.8  & 53.7 \\
\midrule
Transfusion & + Diffusion            & + 1M Image Patches & (+0.3) 10.4 & (+0.2) 6.0 & (-2.0) 51.7 \\
\midrule
Chameleon   & + Stability Modifications & 1M Text Tokens            & (+0.9) 11.0 & (+0.5) 6.3 & (-1.8) 51.9 \\
            & + LM Loss on Image Tokens & + 1M Image Tokens & (+0.8) 11.8 & (+0.5) 6.8  & (-3.0) 48.9 \\
\bottomrule \\
\end{tabular}
\caption{Performance of the 0.76B Transfusion and Chameleon models on text-only benchmarks, compared to the original Llama 2 recipe.}
\label{tab:text_analysis}
\end{table}


\subsection{Architecture Ablations}
\label{sec:ablations}

Now that we have established that Transfusion is a viable, scalable approach to multi-modal modeling in a controlled environment, we can explore improvements and extensions that are applicable to Transfusion alone.

\subsubsection{Attention Masking}
\label{sec:attention}

We first examine the necessity of intra-image bidirectional attention.
Table~\ref{tab:attention} shows that enabling this attention pattern beyond the standard causal attention is advantageous throughout all benchmarks, and using both image encoding/decoding architectures.
In particular, we notice a significant improvement in FID when using linear encoding layers (61.3$\rightarrow$20.3).
In the causal-only version of this architecture, there is no flow of information from patches that appear later in the sequence to those before;
since U-Net blocks contain bidirectional attention within, independent of the transformer's attention mask, this gap is less pronounced when they are applied.

\begin{table}[t]
\small
\centering
\begin{tabular}{@{}llrrrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{Enc/Dec}} & \multirow{2}{*}{\textbf{Attention}} & \multicolumn{1}{c}{\textbf{C4}} & \multicolumn{1}{c}{\textbf{Wiki}} & \multicolumn{1}{c}{\textbf{Llama}} & \multicolumn{3}{c}{\textbf{MS-COCO}} \\
& & \textbf{PPL} ($\downarrow$) & \textbf{PPL} ($\downarrow$) & \textbf{Acc} ($\downarrow$) & \textbf{CDr} ($\uparrow$) & \textbf{FID} ($\downarrow$) & \textbf{CLIP} ($\uparrow$) \\
\midrule
\multirow{2}{*}{Linear} & Causal & 10.4 & 6.0 &  51.4 & 12.7 & 61.3 & 23.0 \\
& Bidirectional & 10.4 & 6.0 & 51.7 & 16.0 & 20.3 & 24.0 \\
\midrule
\multirow{2}{*}{U-Net} & Causal & 10.3 & 5.9  &  52.0 & 23.3 &16.8 & 25.3 \\
& Bidirectional & 10.3 & 5.9 &  51.9 & 25.4 & 16.7 & 25.4 \\
\bottomrule \\
\end{tabular}
\caption{Performance of 0.76B Transfusion models with and without intra-image bidirectional attention. Patch size is set at 2$\times$2 latent pixels.}
\label{tab:attention}
\end{table}

\subsubsection{Patch Size}
\label{sec:patch}

Transfusion models can be defined over different sizes of latent pixel patches.
Larger patch sizes allow the model to pack more images in each training batch and dramatically reduce inference compute, but may come at a performance cost.
Table~\ref{tab:patch_size} sheds light on these performance trade-offs.
While performance does decrease consistently as each image is represented by fewer patches with linear encoding, models with U-Net encoding benefit from larger patches on tasks involving the image modality.
We posit that this is due to the greater amount of total images (and diffusion noise) seen during training. 
We also observe that text performance deteriorates with larger patches, perhaps because transfusion needs to exert more resources (i.e. parameters) to learn how to process images with fewer patches and thus less inference compute.

\begin{table}[t]
\small
\centering
\begin{tabular}{@{}lcccrrrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{Enc/Dec}} & \textbf{Latent/} & \textbf{Pixel/} & \textbf{Patch/} & \multicolumn{1}{c}{\textbf{C4}} & \multicolumn{1}{c}{\textbf{Wiki}} & \multicolumn{1}{c}{\textbf{Llama}} & \multicolumn{3}{c}{\textbf{MS-COCO}} \\
& \textbf{Patch} & \textbf{Patch} & \textbf{Image} & \textbf{PPL} ($\downarrow$) & \textbf{PPL} ($\downarrow$) & \textbf{Acc} ($\downarrow$) & \textbf{CDr} ($\uparrow$) & \textbf{FID} ($\downarrow$) & \textbf{CLIP} ($\uparrow$) \\                 
\midrule
None & 1$\times$1  & 8$\times$8 & 1024 & \textbf{10.3} & \textbf{5.9}  & \textbf{52.2}  & 12.0    &    21.0         & 24.0   \\
\midrule
\multirow{3}{*}{Linear}  & 2$\times$2 & 16$\times$16 & ~~256 & \underline{10.4} & \underline{6.0}    & \underline{51.7}  & \underline{16.0}    & \underline{20.3}        & \underline{24.0}   \\
                       & 4$\times$4  & 32$\times$32 & ~~~~64 & 10.9 & 6.3  & 49.8  & 14.3  & 25.6        & 22.6 \\
                       & 8$\times$8  & 64$\times$64 & ~~~~16 & 11.7 & 6.9  & 47.7  & 11.3  & 43.5        & 18.9 \\
\midrule
\multirow{3}{*}{U-Net} & 2$\times$2 & 16$\times$16 & ~~256 & \textbf{\underline{10.3}} & \textbf{\underline{5.9}}  & \underline{51.9}  & 25.4  & 16.7        & 25.4 \\
                       & 4$\times$4  & 32$\times$32 & ~~~~64 & 10.7 & 6.2  & 50.7  & \textbf{\underline{29.9}}  & \textbf{\underline{16.0}} & \textbf{\underline{25.7}} \\
                       & 8$\times$8 & 64$\times$64 & ~~~~16
                       & 11.4 & 6.6  & 49.2  & 29.5  & 16.1        & 25.2 \\
\bottomrule \\
\end{tabular}
\caption{Performance of 0.76B Transfusion models with different patch sizes. Bolded figures indicate global best, underlines indicate best within architecture.}
\label{tab:patch_size}
\end{table}

\subsubsection{Patch Encoding/Decoding Architecture}
\label{sec:architecture}

Our experiments so far indicate an advantage to using the U-Net up and down blocks instead of a simple linear layer.
One possible reason is that the model benefits from the inductive biases of the U-Net architecure;
an alternative hypothesis is that this advantage stems from the significant increase in overall model parameters introduced by the U-Net layers.
To decouple these two confounders, we scale up the core transformer to 7B parameters, while keeping the amount of U-Net parameters (almost) constant;\footnote{While we do not scale the U-Net layers with the transformer in these experiments, this is a potentially fruitful avenue for future research.}
in this setting, the additional encoder/decoder parameters account for only a 3.8\% increase of total model parameters, equivalent to the amount of token embedding parameters.

Table~\ref{tab:patch_arch} shows that even though the relative benefit of U-Net layers shrinks as the transformer grows, it does not diminish.
In image generation, for example, the U-Net encoder/decoder allows much smaller models to obtain better FID scores than the 7B model with linear patchification layers.
We observe a similar trend in image captioning, where adding U-Net layers boosts the CIDEr score of a 1.4B transformer (1.67B combined) beyond the performance of the linear 7B model.
Overall, it appears that there are indeed inductive bias benefits to U-Net encoding and decoding of images beyond the mere addition of parameters.

\begin{table}[t]
\small
\centering
\begin{tabular}{@{}llcrrrrrr@{}}
\toprule
\textbf{Model} & \multirow{2}{*}{\textbf{Enc/Dec}} & \textbf{$\Delta$ Enc/Dec} & \multicolumn{1}{c}{\textbf{C4}} & \multicolumn{1}{c}{\textbf{Wiki}} & \multicolumn{1}{c}{\textbf{Llama}} & \multicolumn{3}{c}{\textbf{MS-COCO}} \\
\textbf{Params} &  & \textbf{Params} & \textbf{PPL} ($\downarrow$) & \textbf{PPL} ($\downarrow$) & \textbf{Acc} ($\uparrow$) & \textbf{CDr} ($\uparrow$) & \textbf{FID} ($\downarrow$) & \textbf{CLIP} ($\uparrow$) \\
\midrule
\multirow{2}{*}{0.16B} & Linear & ~~~~0.5\% & 14.8 &	8.8	 &  44.2  &  6.2 & 37.6 & 20.0\\
                       & U-Net  & 106.1\%   & 14.4 &	8.5	 &  45.7  &  15.3 &	18.8 & 23.9\\
\midrule
\multirow{2}{*}{0.37B} & Linear & ~~~~0.4\% & 12.0 &	7.0	 &  47.9  &  11.1 &	21.5 & 22.4 \\
                       & U-Net  & ~~71.3\%  & 11.8 &	 6.9  &  48.8  &  21.1 & 18.1 & 24.9 \\
\midrule
\multirow{2}{*}{0.76B} & Linear & ~~~~0.4\% & 10.4 &	6.0	 &  51.7  &  16.0 &	20.3 & 24.0 \\
                       & U-Net  & ~~35.5\%  & 10.3 &	5.9	 &  51.9  &  25.4 &	16.7 & 25.4\\
\midrule
\multirow{2}{*}{1.4B} & Linear & ~~~~0.4\%  & 9.5	 &  5.4  &	53.8  &  19.1 &	19.4 & 24.3\\
                      & U-Net  & ~~19.3\%   & 9.4  &  5.4  &  53.4  &  28.1 & 16.6 & 25.7\\
\midrule
\multirow{2}{*}{7B}   & Linear & ~~~~0.3\%  & 7.7  &  4.3  &  61.5  &  27.2 &	18.6 & 25.9\\
                      & U-Net  & ~~~~3.8\%  & 7.8  &  4.3  &  61.1  &  33.7 & 16.0 & 26.5\\
\bottomrule \\
\end{tabular}
\caption{Performance of linear and U-Net variants of Transfusion across different model sizes. Patch size is set at 2$\times$2 latent pixels. Model parameters refers to the transformer alone.}
\label{tab:patch_arch}
\end{table}

\subsubsection{Image Noising}
\label{sec:noise}

Our experiments order 80\% of image-caption pairs with the caption first, and the image conditioning on the caption, following the intuition that image generation may be a more data-hungry task than image understanding.
The remaining 20\% of the pairs condition the caption on the image.
However, these images are noised as part of the diffusion objective.
We thus measure the effect of limiting the diffusion noise to a maximum of $t=500$ (half of the noise schedule) in the 20\% of cases where images appear before their captions.
Table~\ref{tab:noise_cap} shows that noise limiting significantly improves image captioning, as measure by CIDEr, while having a relatively small effect (less than 1\%) on other benchmarks.

\begin{table}[t]
\small
\centering
\begin{tabular}{@{}lcrrrrrr@{}}
\toprule
\textbf{Model} & \textbf{Noise} & \multicolumn{1}{c}{\textbf{C4}} & \multicolumn{1}{c}{\textbf{Wiki}} & \multicolumn{1}{c}{\textbf{Llama}} & \multicolumn{3}{c}{\textbf{MS-COCO}} \\
\textbf{Params} & \textbf{Limit} & \textbf{PPL} ($\downarrow$) & \textbf{PPL} ($\downarrow$) & \textbf{Acc} ($\uparrow$) & \textbf{CDr} ($\uparrow$) & \textbf{FID} ($\downarrow$) & \textbf{CLIP} ($\uparrow$) \\
\midrule
\multirow{2}{*}{0.76B} &  & 10.3  & 5.9 &  51.9 &  25.4 & 16.7 & 25.4 \\
 & $\checkmark$ & 10.3  & 5.9 &  52.1 &  \textbf{29.4} & 16.5 & 25.4 \\
\midrule
\multirow{2}{*}{7B}					  &   & 7.8  &  4.3 &  61.1  & 33.7 & 16.0 & 26.5 \\
   & $\checkmark$   & 7.7  &  4.3 &  60.9  & \textbf{35.2} & 15.7 & 26.3 \\
\bottomrule \\
\end{tabular}
\caption{Performance of Transfusion with and without limiting the amount of sampled diffusion noise to a maximum of $t=500$ when images appear before the caption.
The models are U-Net variants encoding 2$\times$2 latent pixel patches.
Metrics that change by over 1\% are bolded.}
\label{tab:noise_cap}
\end{table}


\subsection{Comparison with Image Generation Literature}
\label{sec:enhanced}

Our experiments thus far have covered controlled comparisons with Chameleon and Llama, but we have yet to compare Transfusion's image generation capabilities to those of state-of-the-art image generation models.
To that end, we train a 7B parameter model with U-Net encoding/decoding layers (2$\times$2 latent pixel patches) over the equivalent of 2T tokens, comprising of 1T text corpus tokens and 3.5B images and their captions.
While the Transfusion variant in \S\ref{sec:simple} favored simplicity and experimental control, the design choices and data mixture (\S\ref{sec:setup}) of this variant lean a bit more towards image generation.
Figure~\ref{fig:samples1} and Appendix~\ref{sec:examples_image_generation} showcase generated images from this model.

We compare the performance of our model to reported results of other similar scale image generation models, as well as some publicly available text generating models for reference.
Table~\ref{tab:enhanced-joint} shows that Transfusion achieves similar performance to high-performing image generation models such as DeepFloyd \citep{deepfloyd}, while surpassing previously published models including SDXL \citep{podell2023sdxl}.
While Transfusion does lag behind SD 3 \citep{esser2024scaling}, this model leveraged synthetic image captions through backtranslation \citep{dalle3}, which enhances its GenEval performance by 6.5\% absolute (0.433$\rightarrow$0.498) at smaller scale; for simplicity, our experimental setup only included natural data.
Finally, we note that our Transfusion model can also generate text, and performs on par with the Llama models, which were trained on the same text data distribution (\S\ref{sec:setup}).

\begin{table}[t]
\small
\centering
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Text}} & \multirow{2}{*}{\textbf{Images}} & \multicolumn{1}{c}{\textbf{Llama}} & \multicolumn{1}{c}{\textbf{COCO}} & \multicolumn{1}{c}{\textbf{Gen}} \\
& \textbf{Params} & \textbf{Tokens} & & \textbf{Acc} ($\uparrow$) & \textbf{FID} ($\downarrow$) & \textbf{Eval} ($\uparrow$) \\
\midrule
Llama 1 \citep{touvron2023llama} & 7B & 1.4T & --- & 66.1 & --- & --- \\
Llama 2 \citep{llama2} & 7B & 2.0T & --- & 66.3 & --- & --- \\
Chameleon \citep{team2024chameleon} & 7B & 6.0T & 3.5B & 67.1 & 26.74~~ & 0.39 \\
\midrule
Imagen \citep{saharia2022photorealistic} & 2.6B + 4.7B$^{*}$ & --- & 5.0B & --- & 7.27 & --- \\
Parti \citep{yu2022scaling} & 20B & --- & 4.8B & --- & $^{r}$7.23~~ & --- \\
SD 1.5 \citep{rombach2022high} & 0.9B + 0.1B$^{*}$ & --- & 4.0B & --- & --- & 0.43 \\
SD 2.1 \citep{rombach2022high} & 0.9B + 0.1B$^{*}$ & --- & 2.3B & --- & --- & 0.50 \\
DALL-E 2 \citep{dalle2diffusion} & 4.2B + 1B$^{*}$ & --- & 2.6B & --- & 10.39~~ & 0.52 \\
SDXL \citep{podell2023sdxl} & 2.6B + 0.8B$^*$ & --- & 1.6B & --- & --- & 0.55 \\
DeepFloyd \citep{deepfloyd} & 5.5B + 4.7B$^{*}$ & --- & 7.5B & --- & 6.66 & 0.61 \\
SD 3 \citep{sd3} & 8B + 4.7B$^{*}$& --- & $^{s}$2.0B~~ & --- & --- & 0.68 \\
\midrule
Transfusion (Ours) & 7.3B & 1.0T & 3.5B & 66.1 & 6.78 & 0.63 \\
\bottomrule \\
\end{tabular}
\caption{Performance of a 7B Transfusion model (U-Net encoder/decoder layers, 2$\times$2 latent pixel patches) trained on the equivalent of 2T tokens, compared to similar scale models in the literature.
Except Chameleon, all the other models are restricted to generating one modality (either text or image).
$^{*}$ Frozen text encoder parameters.
$^{r}$ Parti samples 16 images for every prompt and then reranks with an auxiliary scoring model.
$^s$ SD 3 trains with synthetic caption data, which provides boosts GenEval performance.
}
\label{tab:enhanced-joint}
\end{table}


\subsection{Image Editing}
\label{sec:editing}

Our Transfusion models, which have been pretrained on text-text, image-text, and text-image data, perform well across these modality pairings.
Can these models extend their capabilities to generate images based on other images?
To investigate, we fine-tuned our 7B model (\S\ref{sec:enhanced}) using a dataset of only 8k publicly available image editing examples, where each example consists of an input image, an edit prompt, and an output image.
This approach, inspired by LIMA \citep{zhou2024lima}, allows us to assess how well the model can generalize to image-to-image generation, a scenario not covered during pretraining.

Manual examination of random examples from the EmuEdit test set \citep{sheynin2024emu}, shown in Figure~\ref{fig:edit1} and Appendix~\ref{sec:editing}, reveals that our fine-tuned Transfusion model performs image edits as instructed.
Despite the limitations of this experiment, the findings suggest that Transfusion models can indeed adapt to and generalize across new modality combinations.
We leave further exploration of this promising direction to future research.


==> old_sections/05_related.tex <==
\section{Related Work}

Most existing multi-modal models are built on the idea of attaching two or more modality-specific architectures together, often pretraining each component separately in advance.
State-of-the-art image and video generation models, for instance, use large pretrained text encoders to represent their input prompts in latent space, which can then be used to condition diffusion models \citep{saharia2022photorealistic}.
In fact, recent work fuses representations from multiple off-the-shelf encoders to enhance performance \citep{podell2023sdxl,sd3}.
A similar pattern can be observed in the vision language model literature, where typically a pretrained language model is complemented by pretrained modality-specific encoders/decoders via projection layers to/from the pretrained text space.
Examples include Flamingo \citep{alayrac2022flamingo} and LLaVA \citep{liu2024visual} for visual understanding, GILL \citep{koh2024generating} for visual generation, and DreamLLM \citep{dongdreamllm} for both visual comprehension and generation.
In contrast, Transfusion has one unified architecture learned end-to-end to generate both text and images.

Prior work on end-to-end multi-modal models includes examples such as Fuyu \citep{fuyu-8b}, which uses image patches as inputs for visual understanding, and Chameleon \citep{team2024chameleon}, which converts each image to a sequence of discretized tokens and then trains over the combined text-image token sequences.
However, these approaches are either restricted to input-level multi-modal tasks, or lag behind state-of-the-art models (i.e. diffusion models) in continuous data generation.
Transfusion provides a simple, end-to-end solution to multi-modal learning that understands and generates high-quality multi-modal data.

An interesting area of recent acrive research is the application diffusion models and their generalizations to discrete text generation \citep{Li-2022-DiffusionLM, gat2024discrete}.
However, this approach has yet to achieve the performance and scale of standard autoregressive language models.
Future research in this direction may unlock new ways to fuse discrete and continuous modalities in a single model.




% \paragraph{Multi-Modal Models}
% Most existing multi-modal models are built on top of pre-trained large language models (LLMs), where LLMs serve as a bridge between different modalities. However, this requires loading multiple pre-trained modality-specific encoders/generators to enable perceiving, processing and producing multi-modal data. Usually this is done by learning a projection layer from the other modality to the pre-trained text space. Typical examples include Flamingo~\citep{alayrac2022flamingo} and LLaVA~\citep{liu2024visual} for visual understanding,  GILL~\citep{koh2024generating} for visual generation, and DreamLLM~\citep{dongdreamllm} for both visual comprehension and generation.
% % \todo{We should mention diffusion for text, and explain that they are not SotA.}
% There are also natively~\cz{by natively, I mean early fusion} trained multi-modal models that learn from multi-modal data from scratch, e.g. Fuyu~\citep{fuyu-8b} which uses image patches as inputs for visual comprehension and Chameleon~\citep{team2024chameleon} which learns from discretized image tokens together with text tokens.
% However, they either can only perform input-level multi-modal tasks, or lag behind state-of-the-art models for each multi-modal task.
% Transfusion provides a native and simple solution to multi-modal learning that understands and generates high-quality multi-modal data in an end-to-end fashion.

% \paragraph{Diffusion Models}
% Diffusion models generate data from noise by learning a reverse forward path from noise to data. They have become the state-of-the-art of generative modeling approach for image~\citep{ho2020denoising,saharia2022photorealistic,sd3}, video~\citep{bar2024lumiere} and audio synthesis~\citep{huang2023make}. 
% Diffusion models are also used for text generation~\citep{Li-2022-DiffusionLM, gat2024discrete}, \todo{let's look up a few more examples about text diffusion -- I think this is one of the first things people will think about} however due to lagging behind causal language models, it's not adopted in large scale language model training.
% The advancements in denoising diffusion probabilistic models (DDPMs) have been driven by improved noise schedules~\citep{hoogeboom2023simple,chen2023importance,nichol2021improved}, improved learning objectives~\citep{sd3,lipman2022flow,salimans2022progressive}~\cz{by learning objective, I mean x-prediction, epsilon-prediction, v-prediction these different parameterization forms, and more efficient training techniques like flow-based learining objectives.}, and better sampling algorithms~\citep{ho2022classifier,song2020denoising,song2023consistency}~\cz{by better, I mean efficiency -- reduce number of inference steps and improved techniques -- CFG.}. Diffusion models are often prompted to generate data, e.g. text-to-image or text-to-video generation. The de-facto design choice of conditional diffusion models need to choose strong pre-trained text encoders~\citep{saharia2022photorealistic} to produce the text representations for diffusion model to condition on, and sometimes representations from several text encoders are combined to provide stronger conditions~\citep{podell2023sdxl,sd3} \todo{dan garette acl 2023}. Thus, the diffusion model needs to be coupled with several off-the-shelf pre-trained models to accomplish conditional generation. In contrast, Transfusion is designed in one single unified architecture that autoregressively learns to generate both text and images, enabling flexible and efficient conditioning when generating multi-modality data by using the same autoregressive architecture for continuous predictions.
% % reusing kv-cache for continuous predictions.


% % \todo{We will want to talk about Fuyu/Flamingo/Llava and explain that they only solve input multimodality, not output}

==> old_sections/06_conclusion.tex <==
\section{Conclusion}

This work explores how to bridge the gap between the state of the art in discrete sequence modeling (next token prediction) and continuous media generation (diffusion).
We propose a simple, yet previously unexplored solution: train a single joint model on two objectives, tying each modality to its preferred objective.
Our experiments show that Transfusion scales efficiently, incurring little to no parameter sharing cost, while enabling the generation of any modality.

